$\texttt{SPIN}$: distilling $\texttt{Skill-RRT}$ for long-horizon prehensile and non-prehensile manipulation

Current robots struggle with long-horizon manipulation tasks requiring sequences of prehensile and non-prehensile skills, contact-rich interactions, and long-term reasoning. We present $\texttt{SPIN}$ ($\textbf{S}$kill $\textbf{P}$lanning to $\textbf{IN}$ference), a framework that distills a computationally intensive planning algorithm into a policy via imitation learning. We propose $\texttt{Skill-RRT}$, an extension of RRT that incorporates skill applicability checks and intermediate object pose sampling for solving such long-horizon problems. To chain independently trained skills, we introduce $\textit{connectors}$, goal-conditioned policies trained to minimize object disturbance during transitions. High-quality demonstrations are generated with $\texttt{Skill-RRT}$ and distilled through noise-based replay in order to reduce online computation time. The resulting policy, trained entirely in simulation, transfers zero-shot to the real world and achieves over 80% success across three challenging long-horizon manipulation tasks and outperforms state-of-the-art hierarchical RL and planning methods.

==> algos/Collect_data.tex <==
\begin{algorithm}[H]
\caption{State-Action Collection}\label{algo:Collect_data}
\begin{algorithmic}[1]
\State \textbf{Input:} Skill library ${\mathcal{O}} = \{o_{\text{NP}_1}, o_{\text{NP}_2}, \ldots, o_{\text{NP}_n}, o_{\text{Place}}\}$
\State \textbf{Initialize:} Counter $n \leftarrow 0$, dataset $\mathcal{D} \leftarrow \emptyset$
\While{$n < 500$}
    \State Randomly sample initial $q^\text{obj}_{\text{init}}$ and goal object pose $q^\text{obj}_{\text{goal}}$
    \State Generate skill plan $\tau_{\text{skill}} = \text{Skill-RRT}(q^\text{obj}_{\text{init}}, q^\text{obj}_{\text{goal}}, {\mathcal{O}})$
    \State Replay the skill plan $\tau_{\text{skill}}$ 400 times to obtain full trajectories $\tau_{\text{full}}^{(i)}$ for $i = 1, \ldots, 400$
    \State Compute replay success rate $r = \frac{1}{400} \sum \text{success}(\tau_{\text{full}}^{(i)})$
    \If{$r \geq 0.9$}
        \State \textcolor{red}{Select 30 successful trajectories randomly} from $\{\tau_{\text{full}}^{(i)} \mid \text{success}(\tau_{\text{full}}^{(i)}) = 1\}$
        \State $\mathcal{D} \leftarrow \mathcal{D} \cup \{\text{selected 30 successful trajectories}\}$
        \State $n \leftarrow n + 1$
    \EndIf
\EndWhile
\end{algorithmic}
\end{algorithm}
\begin{flushleft}
\footnotesize
\textbf{Algorithm \ref{algo:Collect_data} Explanation} — The algorithm collects a dataset of successful state-action trajectories. It begins by sampling random initial and goal states and generating a skill plan $\tau_{\text{skill}}$ using the Skill-RRT algorithm. This plan is executed 500 times to generate full trajectories, with the replay success rate $r$ computed as the ratio of successful trajectories. If $r$ is at least 0.9, 30 successful trajectories are randomly selected and added to the dataset $\mathcal{D}$. This process repeats until 1000 sets of successful trajectories are collected.
\end{flushleft}


==> algos/NP_skill_def.tex <==

\noindent\hrulefill

\noindent \textbf{Skill Definition} $K$

\begin{itemize}\label{Def:NP}
    \item \textbf{Goal-conditioned Policy} \(\pi\)

    \begin{itemize}

        \item \(\pi = 
            \begin{cases} 
            \text{pre-contact policy, } \pi_\text{pre}(q_\text{obj}, q'_\text{obj}): Q_\text{obj} \times Q_\text{obj} \rightarrow Q_r\\
            \text{post-contact policy, } \pi_\text{post}(s, q'_\text{obj}): S \times Q_\text{obj} \rightarrow A \\
            \text{connector policy, } \pi_C(s, q'_r): S \times Q_r \rightarrow A

            \end{cases}\)
    \end{itemize}

    % \item \textbf{Region $R \subsetneq Q_\text{obj}$}
    
    \item \textbf{Applicability checker} $\phi: Q_\text{obj} \times Q_\text{obj} \rightarrow \{0, 1\}$

    \begin{itemize}
        \item[] \underline{\textbf{Card Domain}}
        \begin{itemize}
            \item \(\phi_\text{slide}(q_\text{obj}, q'_\text{obj}) = 
            \begin{cases} 
            1, & \text{if } q'_\text{obj} \in \Qobj, \, q_\text{obj} \in \Qobj, R_x(\qobj)=R_x(q'_\text{obj}), \text{ and } R_y(\qobj)=R_y(q'_\text{obj})\\ 
            0, & \text{otherwise.} 
            \end{cases}\)
            \item \(\phi_\text{Place}(\qobj, q'_\text{obj}) = 
            \begin{cases} 
            1, & \text{if } \pi_\text{pre}(q_\text{obj}, q'_\text{obj}) \text{ is collision-free}, \\ 
            0, & \text{otherwise.} 
            \end{cases}\)
        \end{itemize}
        where \( R_x \) and \( R_y \) are notations for the \( x \) and \( y \) axes in the global frame.

        \item[] \underline{\textbf{Bookshelf Domain}}
            \begin{itemize}
                \item \(\phi_\text{topple}(q_\text{obj}, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } q'_\text{obj} \in \Qobj^\text{upper-shelf}, \, q_\text{obj} \in \Qobj^\text{upper-shelf}, R_x(\qobj) = R_x(\qobj'), \text{ and } R_z(\qobj) = R_z(\qobj') \\ 
                0, & \text{otherwise.} 
                \end{cases}\)
                \item \(\phi_\text{push}(q_\text{obj}, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } q'_\text{obj} \in \Qobj^\text{lower-shelf}, \, q_\text{obj} \in \Qobj^\text{lower-shelf}, R_x(\qobj)=R_x(q'_\text{obj}), \text{ and } R_y(\qobj)=R_y(q'_\text{obj})\\ 
                0, & \text{otherwise.} 
                \end{cases}\)

                \item \(\phi_\text{Place}(\qobj, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } \pi_\text{pre}(q_\text{obj}, q'_\text{obj}) \text{ is collision-free}, \\ 
                0, & \text{otherwise.} 
                \end{cases}\)
            \end{itemize}
        where \( R_z \) is a notation for the \( z \) axis in the global frame.

        \item[] \underline{\textbf{Kitchen Domain}}
            \begin{itemize}
                \item \(\phi_\text{sink}(q_\text{obj}, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } q'_\text{obj} \in \Qobj^\text{sink}, \text{ and } \, q_\text{obj} \in \Qobj^\text{sink} \\ 
                0, & \text{otherwise.} 
                \end{cases}\)
                \item \(\phi_\text{l-cupboard}(q_\text{obj}, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } q'_\text{obj} \in \Qobj^\text{l-cupboard}, \, q_\text{obj} \in \Qobj^\text{l-cupboard}, R_x(\qobj)=R_x(q'_\text{obj}), \text{ and } R_y(\qobj)=R_y(q'_\text{obj})\\ 
                0, & \text{otherwise.} 
                \end{cases}\)
                \item \(\phi_\text{r-cupboard}(q_\text{obj}, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } q'_\text{obj} \in \Qobj^\text{r-cupboard}, \, q_\text{obj} \in \Qobj^\text{r-cupboard}, R_x(\qobj)=R_x(q'_\text{obj}), \text{ and } R_y(\qobj)=R_y(q'_\text{obj})\\ 
                0, & \text{otherwise.} 
                \end{cases}\)
                \item \(\phi_\text{Place}(\qobj, q'_\text{obj}) = 
                \begin{cases} 
                1, & \text{if } \pi_\text{pre}(q_\text{obj}, q'_\text{obj}) \text{ is collision-free}, \\ 
                0, & \text{otherwise.} 
                \end{cases}\)
            \end{itemize}

    \end{itemize}

\end{itemize}

\noindent\hrulefill


==> algos/P_skill_def.tex <==
\noindent\hrulefill

\noindent \textbf{Prehensile (P) Skill Definition} $K_{\text{P}}$

\begin{itemize}\label{Def:P}
    \item \textbf{Goal-conditioned Policy $\pi$}
    \begin{itemize}

        \item \(\pi = 
            \begin{cases} 
            \text{pre-contact policy, } \pi_\text{pre}(s.q_\text{obj}, q'_\text{obj}): Q_\text{obj} \times Q_\text{obj} \rightarrow Q_r\\
            \text{post-contact policy, } \pi_\text{post}(s, q'_\text{obj}): S \times Q_\text{obj} \rightarrow A \\
            \text{connector policy, } \pi_C(s, q'_r): S \times Q_r \rightarrow A

            \end{cases}\)
    \end{itemize}

    % \item \textbf{Region $R = Q_\text{obj}$}

    \item \textbf{Applicability checker} $\phi: S \times Q_\text{obj} \rightarrow \{0, 1\}$
    \begin{itemize}
        \item \(\phi(s, q'_\text{obj}) = 
        \begin{cases} 
        1, & \text{if } \pi_\text{pre}(s.q_\text{obj}, q'_\text{obj}) \text{ is collision-free}, \\ 
        0, & \text{otherwise.} 
        \end{cases}\)
    \end{itemize}

\end{itemize}
\noindent\hrulefill

==> algos/connector_def.tex <==
\noindent\hrulefill

\noindent \textbf{Connector Definition} $c$

\begin{itemize}\label{Def:Connector}
    % \item \textbf{Parameters:} $(q^{\text{obj}}, q^{\text{obj}}_\text{sg}, q^{\text{robot}},  d^\text{obj}, d^\text{robot}, \epsilon^\text{obj}, \epsilon^\text{robot})$
    \item \textbf{Parameters:} $(q^{\text{robot}}_\text{sg}, d^\text{robot}, \epsilon^\text{robot} )$
    \item \textbf{Policy:}
        \begin{itemize}
            \item $a \gets \pi^c(s, q^{\text{robot}}_\text{sg})$
        \end{itemize}

    \item \textbf{Success condition:}
    \begin{itemize}
        % \item $d^\text{obj}(q^\text{obj}_\text{sg}, q^\text{obj}_\text{result}) < \epsilon^\text{obj}$
        \item $d^\text{robot}(q^\text{robot}_\text{sg}, \cdot) < \epsilon^\text{robot}$
    \end{itemize}
\end{itemize}
\noindent\hrulefill


==> algos/skill-RRT/GetConnector.tex <==
\begin{algorithm}[H]
\caption{\texttt{GetConnector}}\label{algo:GetConnector}
\begin{algorithmic}[1]

\Procedure{\texttt{GetConnector}}{$K, \mathcal{K}=\{K_\text{P},K_{\text{NP}_1},\dots, K_{\text{NP}_n}\}, C=\{c_\text{P},c_{\text{NP}_1},\dots, c_{\text{NP}_n}\}$}
    \For{$K_\alpha \in \mathcal{K}$}
        \If{$K == K_\alpha$}
            \State \textbf{return} $c_\alpha$
        \EndIf
    \EndFor
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/GetRegion.tex <==
\begin{algorithm}[H]
\caption{\texttt{GetRegion}}\label{algo:GetRegion}
\begin{algorithmic}[1]

\Procedure{\texttt{GetRegion}}{$K, \mathcal{K},\{\mu^i\}_{i=1,\dots, n}$}
    \For{$i = 1$ to $n$}
        \If{$K == K_{\text{NP}_i}$}
            \State \textbf{return} $\mu^i$
        \EndIf
    \EndFor
    \State \textbf{return} $\cup^n_{i=1}\mu^i$
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/Trad_RRT.tex <==
\begin{algorithm}[H]
\caption{RRT Algorithm}
\label{alg:rrt}
\begin{algorithmic}[1]
\Require Initial state $q_\text{init}$, goal state $q_\text{goal}$, maximum iterations $N_\text{max}$
\State Initialize tree $\mathcal{T} \gets \{q_\text{init}\}$
\For{$i \gets 1$ to $N_\text{max}$}
    \State $q_\text{rand} \gets$ \texttt{Sample()} \Comment{Sample a random state}
    \State $q_\text{near} \gets \texttt{NearestNeighbor}(\mathcal{T}, q_\text{rand})$ \Comment{Find nearest node in $\mathcal{T}$}
    \State $q_\text{new} \gets \texttt{Extend}(q_\text{near}, q_\text{rand})$ \Comment{Generate new state}
    \If{$q_\text{new} \in \mathcal{C}_\text{free}$}
        \State Add $q_\text{new}$ to $\mathcal{T}$ with an edge to $q_\text{near}$
    \EndIf
    \If{$q_\text{new} = q_\text{goal}$}
        \State \Return Path from $q_\text{init}$ to $q_\text{goal}$ in $\mathcal{T}$
    \EndIf
\EndFor
\State \Return Failure
\end{algorithmic}
\end{algorithm}

==> algos/skill-RRT/concrete_skill_rrt.tex <==
\begin{algorithm}[H]
\caption{\texttt{Concrete-Skill-RRT}}\label{algo:concrete-skill-rrt}
\begin{algorithmic}[1]

\Procedure{\texttt{Concrete-Skill-RRT}}{$ q^{\text{obj}}_0, q^{\text{robot}}_0, q^{\text{obj}}_{\text{goal}}, \mathcal{O}, \ \ \ \ \ \ $ \hspace*{3em}$ \{\mu^i\}_{i=1, \dots, n}, p_g,$ $d^\text{robot}(\cdot, \cdot), d^\text{obj}(\cdot, \cdot), \epsilon^\text{robot}, \epsilon^\text{obj}, C $}

    \State \textbf{Return} \hyperref[algo:Universal-skill-rrt]{\texttt{Skill-RRT}}$\big( q^{\text{obj}}_0, q^{\text{robot}}_0, q^{\text{obj}}_{\text{goal}}, \mathcal{O}, \{\mu^i\}_{i=1, \dots, n},$
    \hspace*{10em} $p_g,d^\text{robot}(\cdot, \cdot), d^\text{obj}(\cdot, \cdot), \epsilon^\text{robot}, \epsilon^\text{obj},$ 
    \hspace*{7em} \hyperref[algo:Extend]{\texttt{ConcreteExtend}}$(\cdot, \cdot,\cdot, \cdot,\cdot, \cdot,\cdot, \cdot, C) \big)$

\EndProcedure
\end{algorithmic}
\end{algorithm}



==> algos/skill-RRT/extend.tex <==
\begin{algorithm}[H]
\caption{\texttt{ConcreteExtend}}\label{algo:Extend}
\begin{algorithmic}[1]

\Procedure{\texttt{ConcreteExtend}}{$T, v_{\text{near}}, o, {q}^{\text{obj}}_{sg}, d^\text{robot}, d^\text{obj},$ 
\hspace*{18em} $ \epsilon^\text{robot},\epsilon^\text{obj}, C$}
    \State $c \gets \texttt{GetConnector}(o,, \mathcal{O}, C)$
    \State ${q}^{\text{robot}}_{\text{sg}} \gets o.\pi^{\text{pre}}(v_{\text{near}}.q^{\text{obj}}_\text{pose}, {q}^{\text{obj}}_{sg})$
    \State $(q^{\text{obj}}_\text{pose})^c,(q^{\text{obj}}_\text{vel})^c, (q^{\text{robot}}_\text{pos})^c, (q^{\text{robot}}_\text{vel})^c \gets \texttt{simulate}( c.\pi^{c}$
    
    \hspace*{16.5em}$, v_{\text{near}}, {q}^{\text{robot}}_{\text{sg}})$

    \If{$\textbf{not } d^\text{robot}((q^\text{robot}_\text{pos})^c, q^\text{robot}_\text{sg}) < \epsilon^\text{robot}$}
        \State \Return $T$
    \EndIf

    \State ${v^c_{\text{new}}} \gets \{c, q^{\text{robot}}_\text{sg}, (q^{\text{obj}}_\text{pose})^c,(q^{\text{obj}}_\text{vel})^c, (q^{\text{robot}}_\text{pos})^c, (q^{\text{robot}}_\text{vel})^c\}$

    \State $q^{\text{obj}}_\text{pose},q^{\text{obj}}_\text{vel}, q^{\text{robot}}_\text{pos}, q^{\text{robot}}_\text{vel} \gets \texttt{simulate}(o.\pi, v^c_\text{new}, {q}^{\text{obj}}_{sg})$

    \If{\textbf{not} $d^\text{obj}({q}^{\text{obj}}_\text{pose}, {q}^{\text{obj}}_{sg}) < \epsilon^\text{obj} $}
        \State \Return $T$
    \EndIf

    \State ${v_{\text{new}}} \gets \{o, q^\text{obj}_{sg}, q^{\text{obj}}_\text{pose},q^{\text{obj}}_\text{vel}, q^{\text{robot}}_\text{pos}, q^{\text{robot}}_\text{vel}\}$
    \State $T$.AddNodes$({v}_{\text{new}})$
    \State $T$.AddNodes$({v}^c_{\text{new}})$

    \State $v_{\text{new}}.\text{parent} = v^c_{\text{new}}$
    \State $v^c_{\text{new}}.\text{parent} = v_{\text{near}}$

    \State \Return $T$
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/extend_abstract.tex <==
\begin{algorithm}[H]
\caption{\texttt{LazyExtend}}\label{algo:AbstractExtend}
\begin{algorithmic}[1]

\Procedure{\texttt{LazyExtend}}{$T$, $v_{\text{near}}$, $o$, ${q}^{\text{obj}}_{sg}, d^\text{obj}, \epsilon^\text{obj}$}
    \State ${q}^{\text{robot}}_{\text{pre}} \gets o.\pi^\text{pre}(v_{\text{near}}.q^{\text{obj}}_\text{pose}, {q}^{\text{obj}}_{sg})$
    \State $v^c_\text{new} \gets \{\emptyset, q^\text{robot}_\text{pre},v_\text{near}.q^\text{obj}_\text{pose},v_\text{near}.q^\text{obj}_\text{vel},q^\text{robot}_\text{pre}, \textbf{0} \}$ % \Comment{Teleport $q^\text{robot}$}
    \State \Comment{Teleport $q^\text{robot}_\text{pos}$ to $q^\text{robot}_\text{pre}$}
    \State $q^{\text{obj}}_\text{pose},q^{\text{obj}}_\text{vel}, q^{\text{robot}}_\text{pos}, q^{\text{robot}}_\text{vel} \gets \texttt{simulate}(o.\pi, v^c_\text{new}, {q}^{\text{obj}}_{sg})$
    \If{\textbf{not} $d^\text{obj}({q}^{\text{obj}}_\text{pose}, {q}^{\text{obj}}_{sg}) < \epsilon^\text{obj} $}
        \State \Return $T$
    \EndIf

    \State ${v_{\text{new}}} \gets \{o, q^\text{obj}_{sg}, {q}^{\text{obj}}_\text{pose},{q}^{\text{obj}}_\text{vel}, {q}^{\text{robot}}_\text{pose},  {q}^{\text{robot}}_\text{vel}\}$
    \State $T$.AddNodes$({v}_{\text{new}})$
    \State $T$.AddNodes$({v}^c_{\text{new}})$
    \State $v_{\text{new}}.\text{parent} = v^c_{\text{new}}$
    \State $v^c_{\text{new}}.\text{parent} = v_{\text{near}}$
    \State \Return $T$
\EndProcedure

\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/gpusampleskillandsubgoal.tex <==
\begin{algorithm}[H]
\caption{\texttt{BatchedUnifSmplSkillAndSubgoal}($\mathcal{K}, q^g_\text{obj}, p_g$)}\label{algo:UnifSmplSkillAndSubgoal}
\begin{algorithmic}[1]

\State $K \gets \text{BatchedUniformSample}(\mathcal{K})$
\State $p \leftarrow \text{rand}(1)$ 
\If{$p < p_g$}
    \State $q_{\text{obj}} \gets q^{g}_\text{obj}$
\Else
    \State $q_{\text{obj}} \gets \text{BatchedUniformSamplePose}(K.R)$
\EndIf

\State \Return $K, q_{\text{obj}}$

\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/lazy_skill_rrt.tex <==
\begin{algorithm}[H]
\caption{\texttt{Lazy-Skill-RRT}}\label{algo:lazy-skill-rrt}
\begin{algorithmic}[1]

\Procedure{\texttt{Lazy-Skill-RRT}}{$q^{\text{obj}}_0, q^{\text{robot}}_0, q^{\text{obj}}_{\text{goal}}, \mathcal{O}, \ \ \ \  $ \hspace*{4.5em} $ \{\mu^i\}_{i=1, \dots, n}, p_g, d^\text{robot}(\cdot, \cdot), d^\text{obj}(\cdot, \cdot), \epsilon^\text{robot}, \epsilon^\text{obj} $}

    \State \textbf{Return} \hyperref[algo:Universal-skill-rrt]{\texttt{Skill-RRT}}$\big( q^{\text{obj}}_0, q^{\text{robot}}_0,  q^{\text{obj}}_{\text{goal}}, \mathcal{O}, \{\mu^i\}_{i=1, \dots, n}, $ 
    \hspace*{1cm} $p_g, d^\text{robot}(\cdot, \cdot), d^\text{obj}(\cdot, \cdot), \epsilon^\text{robot}, \epsilon^\text{obj},$
    \hspace*{11em} \hyperref[algo:AbstractExtend]{\texttt{LazyExtend}}$(\cdot, \cdot,\cdot, \cdot,\cdot, \cdot,\cdot, \cdot) \big)$

\EndProcedure
\end{algorithmic}
\end{algorithm}


==> algos/skill-RRT/skill-rrt_abstract.tex <==
\begin{algorithm}[H]
\caption{\texttt{Abstract-Skill-RRT}}\label{algo:Abstract-skill-rrt}
\begin{algorithmic}[1]
\State \textbf{Input:} initial and goal config $(q^{\text{obj}}_0, q^{\text{obj}}_{\text{goal}})$, skill library $\mathcal{O}$ \\
Metric function $d$ to calculate distance between object poses, Goal sample probability $p_g$

\State $T=\emptyset$    \Comment{Initialize empty tree}
\State $v_{0} \gets \{ q^{\text{obj}}_{0}\}$ \Comment{Create a start node}
% \State $v_\text{goal} \gets \{ q^{\text{obj}}_\text{goal}\}$ \Comment{Create a goal node}
\State $T$.AddNode($v_{0}$)

\While{True}
    \State ${o_\alpha}, {q}^{\text{obj}}_{sg} \gets $\hyperref[algo:SampleSkillAndPose]{\texttt{SampleSkillAndSubgoal}}($\mathcal{O}, p_g$)
    \State ${v}_{\text{near}} \gets$ \hyperref[algo:NearestNode]{\texttt{CheckPreAndNearestNode}}($T, o_\alpha, q^{\text{obj}}_{sg}, d$)
    \State $T \leftarrow $ \hyperref[algo:AbstractExtend]{\texttt{AbstractExtend}}$(T, v_{\text{near}}, o_\alpha, {q}^{\text{obj}}_{sg})$
    \If{$q^{\text{obj}}_{\text{goal}} \in \bigcup_{v \in T.V} \{ v.q^{\text{obj}}_{\text{sg}} \}$}
        \State $v_{\text{goal}} \gets v \in T.V \ \text{s.t.} \ v.q^{\text{obj}}_{\text{sg}} = q^{\text{obj}}_{\text{goal}}$
        \State \textbf{break}
    \EndIf
\EndWhile

\State $\tau^\text{abstract}_{\text{skill}} \gets []$ \Comment{Initialize an empty list}
\While{$v_{\text{goal}} \neq v_0$}
    \State $\tau^\text{abstract}_{\text{skill}}.\text{append}(v_{\text{goal}})$
    \State $v_{\text{goal}} \gets v_{\text{goal}}.\text{parent}$
\EndWhile
\State $\tau^\text{abstract}_{\text{skill}} \gets \tau^\text{abstract}_{\text{skill}}[::-1]$ \Comment{Reverse the list}
\State \Return $\tau^\text{abstract}_{\text{skill}}$

\end{algorithmic}
\end{algorithm}
% {\footnotesize
%\textbf{Algorithm \ref{algo:skill-rrt} Explanation} — The Skill-RRT algorithm plans a path from an initial configuration $(q^{\text{obj}}_0, q^{\text{robot}}_0)$ to a goal configuration $q^{\text{obj}}_{\text{goal}}$ using a library of skills $\mathcal{O}$ and connectors $C$. It initializes a tree $T$ with the start node $v_0$ and iteratively samples skills and subgoal configurations. The nearest feasible node in $T$ is identified, and the tree is extended toward the subgoal with skill simulation. If the goal configuration is reached within $N_{max}$ attempts, the path is returned; otherwise, the algorithm fails.}

==> algos/skill-RRT/skill-rrt_whole.tex <==
\begin{algorithm}[H]
\caption{\texttt{Skill-RRT}}\label{algo:skill-rrt}
\begin{algorithmic}[1]
\State \textbf{Input:} initial config $(q^{\text{obj}}_0$, $q^{\text{robot}}_0)$, goal config $q^{\text{obj}}_{\text{goal}}$, \\
skill library $\mathcal{O}=\{o_\alpha \mid \alpha \in \{\text{NP}_1, ..., \text{NP}_n, \text{Place}\}\}$, \\
\colorbox{gray!20}{\makebox[\dimexpr\linewidth-1em\relax][l]{connector library $C=\{c_\alpha \mid \alpha \in \{\text{NP}_1, ..., \text{NP}_n, \text{Place}\}\}$}}, \\
set of regions $\mathcal{M}=\{(\mu^i_{\mathcal{I}}, \mu^i_{\beta}) \mid i \in \{1, ..., n\}\}$, \\
Metric function $d$ to calculate distance between $(q^{\text{obj}}, q^{\text{obj}}_{sg})$, \\ Goal sample probability $p_g$
\State \textbf{Output:} skill plan $\tau_{\text{skill}}$ \\

\State $T=\emptyset$    \Comment{Initialize empty tree}
\State $v_{0} \gets \{ q^{\text{obj}}_{0} \}$ \Comment{Create a start node}
\State $T$.AddNode($v_{0}$)

\While{True}
    \State ${o_\alpha}, {q}^{\text{obj}}_{sg} \gets $\hyperref[algo:SampleSkillAndPose]{\texttt{SampleSkillAndSubgoal}}($\mathcal{O}, p_g$)
    \State ${v}_{\text{near}} \gets$ \hyperref[algo:NearestNode]{\texttt{CheckPreAndNearestNode}}($T, o_\alpha, q^{\text{obj}}_{sg}, d$)
\State \colorbox{gray!20}{\makebox[\dimexpr\linewidth-2em\relax][l]{$T \leftarrow $ \hyperref[algo:Extend]{\texttt{Extend}}$(T, v_{\text{near}}, o_\alpha, c_\alpha, {q}^{\text{obj}}_{sg})$}}
    \If{$q^{\text{obj}}_{\text{goal}} \in \bigcup_{v \in T.V} \{ v.q^{\text{obj}}_{\text{sg}} \}$}
        \State $v_{\text{goal}} \gets v \in T.V \ \text{s.t.} \ v.q^{\text{obj}}_{\text{sg}} = q^{\text{obj}}_{\text{goal}}$
        \State \textbf{break}
    \EndIf
\EndWhile

\State $\tau^\text{full}_{\text{skill}} \gets []$ \Comment{Initialize an empty list}
\While{$v_{\text{goal}} \neq v_0$}
    % \If{$v_{\text{goal}}.\text{type} == \text{skill}$}
    %     \State \colorbox{gray!20}{\makebox[\dimexpr\linewidth-3.5em\relax][l]{$\tau_{\text{skill}}.\text{append}((v_{\text{goal}}.o, v_{\text{goal}}.q^\text{obj}_\text{sg}))$}}
    % \Else
    %     \State \colorbox{gray!20}{\makebox[\dimexpr\linewidth-3.5em\relax][l]{$\tau_{\text{skill}}.\text{append}((v_{\text{goal}}.c, v_{\text{goal}}.q^\text{robot}_\text{pre}))$}}
    % \EndIf
    \State $\tau^\text{full}_{\text{skill}}.\text{append}(v_{\text{goal}})$
    \State $v_{\text{goal}} \gets v_{\text{goal}}.\text{parent}$
\EndWhile

\State $\tau^\text{full}_{\text{skill}} \gets \tau^\text{full}_{\text{skill}}[::-1]$ \Comment{Reverse the list}
\State \Return $\tau^\text{full}_{\text{skill}}$

\end{algorithmic}
\end{algorithm}



==> algos/skill-RRT/skill_rrt.tex <==
\begin{algorithm}[H]
\caption{\texttt{Skill-RRT}}\label{algo:Universal-skill-rrt}
\begin{algorithmic}[1]

\Procedure{\texttt{Skill-RRT}}{
  $q^{\text{obj}}_0, q^{\text{robot}}_{0}, q^{\text{obj}}_{\text{goal}}, \mathcal{O},\{\mu^i\}_{i=1, \dots, n}$, 
  \hspace{1cm} $p_g$, $d^\text{robot}(\cdot, \cdot)$, $d^\text{obj}(\cdot, \cdot)$, 
  $\epsilon^\text{robot}$, $\epsilon^\text{obj}$, \texttt{Extend}$(\cdot, \cdot, \cdot, \cdot, \cdot, \cdot, \cdot, \cdot)$
}

\State $T=\emptyset$   \Comment{Initialize an empty tree}
\State $v_{0} \gets \{\emptyset, \emptyset,  q^{\text{obj}}_{0},  \textbf{0},q^\text{robot}_0,  \textbf{0}\}$ \Comment{Root: no skill, subgoal}
\State $v_\text{goal} \gets $ None
\State $T$.AddNode($v_{0}$)

\For{$i = 1$ \textbf{to} $N$}
    \State ${o}, {q}^{\text{obj}}_{sg} \gets $\hyperref[algo:SampleSkillAndPose]{\texttt{SampleSkillSubgoal}}($\mathcal{O}, p_g, \ \ \ \ \ \ $
    \hspace*{18em}$ \{\mu^i\}_{i=1, \dots, n}$)
    \State ${v}_{\text{near}} \gets$ \hyperref[algo:NearestNode]{\texttt{GetFeasibleNearestNode}}($T, o, q^{\text{obj}}_{sg},$
    \hspace*{21.5em}$ d^\text{obj}$)
    \If{$v_\text{near}$ is $\emptyset$} 
        \State \textbf{continue}
    \EndIf
    \State $T \leftarrow $ \texttt{Extend}$\big(T, v_{\text{near}}, o, q^{\text{obj}}_{sg}, d^\text{robot}(\cdot, \cdot), d^\text{obj}(\cdot, \cdot),$ \\
    \hspace*{19em} $ \epsilon^\text{robot}, \epsilon^\text{obj}\big)$
    \If{$q^{\text{obj}}_{\text{goal}} \in \bigcup_{v \in T.V} \{ v.q^{\text{obj}}_{\text{sg}} \}$}
        \State $v_{\text{goal}} \gets v \in T.V \ \text{s.t.} \ v.q^{\text{obj}}_{\text{sg}} = q^{\text{obj}}_{\text{goal}}$
        \State \textbf{break}
    \EndIf
\EndFor

\If{$v_\text{goal}$ is None}
    \State \textbf{Return} None
\Else
    \State $\texttt{Path}_{\text{skill}} \gets \texttt{Retrace}(v_\text{goal}) $
    \State \textbf{Return} $\texttt{Path}_{\text{skill}}$
\EndIf
\EndProcedure

\Statex
\hrulefill


\end{algorithmic}
\end{algorithm}

==> algos/skill_feasibility_reject.tex <==

\noindent\hrulefill

\noindent \textbf{non-prehensile (NP) Skill feasibility rejection rule}

\begin{itemize}\label{Feasible_rejection:NP}
    \item \textbf{Feasibility rejection rule:}
    \begin{enumerate}
        \item \texttt{IKFeasible}($ \pi^\text{pre}_{\text{NP}_i}(q^\text{obj}, q^\text{obj}_\text{sg})$) \\ $(q^\text{obj} \in \mu^i)$ \\ $(q^\text{obj}_\text{sg} \in \mu^i)$  
        % \item $d^\text{robot}\big( q^\text{robot}, \pi^\text{pre}_{\text{NP}_i}(q^\text{obj}, q^\text{obj}_\text{sg}) \big) < \epsilon^\text{robot}$
    \end{enumerate}

\end{itemize}

\noindent\hrulefill

\noindent\hrulefill

\noindent \textbf{prehensile (P) Skill feasibility rejection rule}

\begin{itemize}\label{Feasible_rejection:P}
    \item \textbf{Feasibility rejection rule:}
    \begin{enumerate}
        \item \texttt{IKFeasible}($ \pi^\text{pre}_\text{P}(q^\text{obj}, q^\text{obj}_\text{sg})$) % \\ \texttt{IKFeasible}($ \pi^\text{pre}_\text{P}(q^\text{obj}_\text{sg}, q^\text{obj})$) 
        % \item $d^\text{robot}\big( q^\text{robot}, \pi^\text{pre}_\text{P}(q^\text{obj}, q^\text{obj}_\text{sg}) \big) < \epsilon^\text{robot}$
    \end{enumerate}    
\end{itemize}
\noindent\hrulefill

==> algos/train_connector_NP.tex <==
\begin{algorithm}[H]
\caption{Training Connector Policy $\pi^c_{\text{NP}_i}$ for Non-Prehensile Skill $\kappa_{\text{NP}_i}$}\label{algo:train_connector_NP}
\begin{algorithmic}[1]
\State Initialize dataset $\mathcal{D} \leftarrow \emptyset$
\While{$|\mathcal{D}| < 1000$}
    \State Sample $q^O$ from $\mathcal{M}$ and $q^O_{\text{sg}}$ from $\mu_i$
    \If{$\text{precondition}^0_{\text{Place}}(q^O, q^O_{\text{sg}})$}
        \State $q^R_{\text{pre}} = f^{\text{pre}}(q^O, q^O_{\text{sg}})$
        \State $q^O_{\text{final}}, q^R_{\text{final}} \leftarrow \mathcal{T}_{simul}(\pi_{\text{Place}}, q^O, q^R_{\text{pre}}, q^O_{\text{sg}})$
        \If{CheckSuccess($q^O_{\text{final}}, q^O_{sg}$)}
            \State $(q^O_{\text{sg}})_i \leftarrow \text{UniformSamplePose}(\mu_i)$
            \If{ $\text{precondition}^0_{\text{NP}_i}( q^O_{\text{final}}, (q^O_{\text{sg}})_i)$}
                \State $(q^R_{\text{pre}})_i = f^{\text{pre}}_{\text{NP}_i}(q^O_{\text{final}}, ({q^O_{\text{sg}})_i})$
                \State Add $((q^O_{\text{final}}, q^R_{\text{final}}), (q^R_{\text{pre}})^i)$ to $\mathcal{D}$
            \EndIf
        \EndIf
    \EndIf
\EndWhile
\State Train $\pi^c_{\text{NP}_i}$ with $\mathcal{D}$ using PPO
\end{algorithmic}
\end{algorithm}


==> algos/train_connector_P.tex <==
\begin{algorithm}[H]
\caption{Training Connector Policy $\pi^c_{\text{Place}}$ for Place Skill $\kappa_{\text{Place}}$}\label{algo:train_connector_P}
\begin{algorithmic}[1]
\State Initialize dataset $\mathcal{D_{\text{final}}} \leftarrow \emptyset$
\State Initialize dataset $\mathcal{D} \leftarrow \emptyset$
\While{$|\mathcal{D}| < 1000$}
    \For{each Non-Prehensile skill $\kappa_{\text{NP}_i}$}
        \State $q^O \leftarrow \text{UniformSamplePose}(\mu_i)$
        \State $q^O_{\text{sg}} \leftarrow \text{UniformSamplePose}(\mu_i)$
        \If{$\text{precondition}^0_{\text{NP}_i}(q^O, q^O_{\text{sg}})$}
            \State $q^R_{\text{pre}} = f^{\text{pre}}_{\text{NP}_i}(q^O, q^O_{\text{sg}})$
            \State $q^O_{\text{final}}, q^R_{\text{final}} \leftarrow \mathcal{T}_{simul}(\pi_{\text{NP}_i}, q^O, q^R_{\text{pre}}, q^O_{\text{sg}})$
            \If{CheckSuccess($q^O_{\text{final}}, q^O_{\text{sg}}$)}
                \State Add $(q^O_{\text{final}}, q^R_{\text{final}})$ to $\mathcal{D_{\text{final}}}$
            \EndIf
        \EndIf
    \EndFor
    \State Sample $(q^O_{\text{final}}, q^R_{\text{final}})$ from $\mathcal{D_{\text{final}}}$
    \State Sample $(q^O_{sg})_{\text{place}}$ from $\mathcal{M}$
    \If{$\text{precondition}^0_{\text{Place}}(q^O_{\text{final}}, (q^O_{sg})_{\text{place}})$}
        \State $(q^R_{\text{pre}})_{\text{place}} = f^{\text{pre}}_{\text{place}}(q^O_{\text{final}}, (q^O_{sg})_{\text{place}})$
        \State Add $((q^O_{\text{final}}, q^R_{\text{final}}), (q^R_{\text{pre}})_{\text{place}})$ to $\mathcal{D}$
    \EndIf
\EndWhile
\State Train $\pi^c_{\text{Place}}$ with $\mathcal{D}$ using PPO
\end{algorithmic}
\end{algorithm}

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne '') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> sections/01_intro_old.tex <==
% Task motivation + our ultimate goal
Humans have a remarkable capability to use sequences of prehensile (P) and non-prehensile (NP) manipulation in everyday life. For example, to take a book from a crowded shelf and place it in a tight space where our entire hand would not fit, we topple the book to enable grasping, pick-and-place it to the edge of the target space, and then push it into place using just our fingers. Our ultimate goal is to develop a policy that allows robots to solve such \textit{\textbf{p}rehensile–\textbf{n}on‑\textbf{p}rehensile (PNP)} tasks that require moving an object from a random initial state to a random target pose using a sequence of P and NP manipulations, as illustrated in Figure~\ref{fig:CPNP_tasks}. Such problems are extremely complex: they demand reasoning not just about the feasibility of each skill but also how to \textit{chain} them, such as toppling a book to enable a later grasp.
	
\begin{figure}[htb]
\includegraphics[width=\textwidth]{figures/figure_task_v2.png}
\captionof{figure}{\label{fig:CPNP_tasks} Overview of our tasks. The first column shows objects. Yellow and green lines mark the initial and goal object poses in the second column. (First row) the robot must flip a thin card initially in an ungraspable pose by first moving it to the end of the table, flipping it, and putting it in the target pose. (Second row) the robot must put it in the lower shelf where the robot gripper cannot fit by first toppling the book, picking and placing it to the end of the lower shelf and then pushing it inside. (Third row) the robot must upright the cup in a sink, grab it, place it on the cupboard, and ensure the handle is inside the desired region by re-orienting it. The red arrow indicates the movement of the object, while the orange arrow represents the movement of the robot. We highly recommend our supplementary video.}
\end{figure}

One way to address this problem is learning‑based approaches, particularly reinforcement learning (RL) and imitation learning (IL), which have shown promise in recent years~\cite{kalashnikov2018scalable, handa2023dextreme, cho2024corn, chen2023visual, chi2023diffusion, fu2024mobile, Reuss-RSS-23, wang2023mimicplay, Zhao-RSS-23}. However, PNP problems require reasoning over a large number of actions (e.g., more than 500 joint torques) and RL struggles with such long‑horizon tasks~\cite{andrychowicz2021matters}. These issues are especially pronounced in our tasks, where the object must temporally move away from the goal before ultimately reaching it, such as sliding a card to the edge of a table before grasping it (Figure~\ref{fig:CPNP_tasks}, top row). IL, in contrast, sidesteps the exploration challenge through dense supervision from human demonstrations. However, it scales poorly to the wide variety of initial states and goals, because collecting such large‑scale, long‑horizon demonstrations is expensive~\cite{fu2024mobile, chi2024universal, lin2024learning}. 

\iffalse
\emph{Temporal abstraction} alleviates the challenges of RL by allowing a high-level policy to plan over extended segments of behavior, while a reusable low-level policy handles short-horizon primitive actions~\cite{sutton1999between}. 
%To exploit such temporally extended actions, often called skills or options, 
Prior work such as hierarchical RL (HRL) has investigated hierarchical architectures to exploit such temporally extended actions~\cite{nachum2018data,lee2019composing, lee2019learning, zhang2022adjacency,wang2024probabilistic}.
%This hierarchy enables the high‑level policy to focus on long‑term plans, thereby reducing the search space and easing the exploration burden. 
However, jointly learning high-level and low-level policies is often unstable because every update to a low‑level policies shifts the dynamics observed by the high-level policy~\cite{nachum2018data, gurtler2021hierarchical}.%, turning the high-level policy’s optimization into a moving target~\cite{}.
\fi

% Motivation of utilizing already trained skills + TAMP/PAMDP limitations
Rather than operating in a low-level action space such as joint torques, we propose to use temporally-abstracted skills to solve PNP problems. Specifically, we propose to leverage the P and NP skill learning algorithms to independently train the skills, and chain them together to solve PNP problems~\cite{mahler2017dex, joshi2020robotic, sundermeyer2021contact, fang2023anygrasp, zhou2023learning, kim2023pre, zhou2023hacman, cho2024corn}. 
We assume each skill consists of a \emph{goal-conditioned policy} that takes as an input a desired object pose and outputs a sequence of joint torques to achieve that pose, and an \emph{applicability checker} which, given a state, checks whether the skill can be applied in that state.

%This reduces our challenge to finding just a high‑level policy that effectively chains these skills. We assume access to a set of independently trained skills, where their training processes do not assume the knowledge of other skills. Each skill consists of a \emph{goal-conditioned policy} that takes as an input a desired object pose and outputs a sequence of joint torques to achieve that pose, and an \emph{applicability checker} which, given a state, checks whether the skill can be applied in that state.

Several approaches have been explored. One avenue is task‑and‑motion planning (TAMP), which has proved effective for long‑horizon problems~\cite{garrett2021integrated}. However, the issue with applying TAMP to PNP problems is that TAMP requires preconditions and effects of a skill, which define the deterministic transition model of the skill but in PNP domains, such information is rarely available because of the following reasons. First, even when the preconditions are satisfied, a skill is not guaranteed to succeed, especially for an NP skill that undergoes numerous contact‑mode transitions during execution. Second, even if the skill succeeds, the outcome is stochastic: the object ends up at a random pose within some proximity of the target pose, rather than exactly at the target pose. 
Another line of work frames the problem as a parameterized‑action Markov decision process (PAMDPs)~\cite{hausknecht2015deep, xiong2018parametrized, li2021hyar, dalal2021accelerating, nasiriany2022augmenting}, where each action is a skill described by a discrete index and a continuous parameter vector, and then solves the problem with RL. In this method, deterministic transition models for each skill are not necessarily required. Yet PAMDPs with RL still struggle with exploration when a carefully shaped reward function is unavailable.

% In this paper,
% For aforementioned limitations of skill chaining algorithms,
Instead, we propose a two-stage framework: (1) a planning stage that generates a large number of skill plans (i.e., sequences of skills and their corresponding goals) for PNP problems using an independently trained skill library and a GPU-based simulator; and (2) a distillation stage based on IL to reduce online computation time of planning.

To generate skill plans without preconditions and effects of a skill or a carefully shaped reward function, we propose a novel planner, \texttt{Skill-RRT}, that extends the classical RRT~\cite{lavalle1998rapidly} into the space of skills and object goals. RRT efficiently explores the search space by randomly sampling a robot configuration, extending from the nearest node in the tree if the configuration is collision-free, and rejecting it otherwise. \texttt{Skill-RRT} has the same structure, but introduces three key modifications: (1) instead of sampling a robot configuration, it samples object pose and skill from the space of object poses and the discrete set of skills; (2) it extends from the nearest node in the tree only if the sampled skill is both applicable and succeeds when simulated with the sampled object pose as its goal; and (3) it parallelizes sampling and extending in a GPU-based simulator, significantly accelerating planning. By leveraging RRT's exploration strategy, \texttt{Skill-RRT} facilitates efficient planning in the space of skills and intermediate object poses.

\iffalse
\textcolor{red}{FIX:}
% Skill gap + motion planner limitations
Beyond the limitations of existing approaches, a more fundamental challenge in PNP problems lies in chaining \emph{independently} trained skills (i.e. skills that are unaware of one another) where \textcolor{red}{a large state gap exists between the terminal state of one skill and the initial state of the next~\cite{konidaris2009skill}}. In the card task, for instance, the sliding skill terminates once the robot has positioned the card at its target pose with the gripper closed and resting on top of the card (Figure~\ref{fig:CPNP_tasks}, third column). The subsequent prehensile skill, however, expects the robot to start from a pre‑grasp pose at the side of the card with the gripper open (Figure~\ref{fig:CPNP_tasks}, fourth column). However, this motion belongs to neither the sliding nor the prehensile skill.
\fi

However, a key challenge with \texttt{Skill-RRT} is the presence of a large state gap between skills, as skills are not inherently designed to be chained~\cite{konidaris2009skill}. This state gap refers to the discrepancy between the resulting state of one skill and the applicable states required by the next skill. For example, in the card domain, a sliding skill ends when the robot positions the object at the desired pose, with the gripper closed and positioned on top of the card (Figure~\ref{fig:CPNP_tasks}, third column). To transition to a prehensile skill, the robot must move to a pre-grasp configuration at the side of the card with the gripper opened, as this is the applicable state of the prehensile skill (Figure~\ref{fig:CPNP_tasks}, fourth column). However, this motion belongs to neither the sliding nor the prehensile skill. One na\"ive solution is to use a collision-free motion planner to move the gripper, but we found that this approach often fails because control errors can disturb the object and cause it to fall, or small object movements due to unstable poses can invalidate the planned collision-free path.

To address this state gap, we introduce \textit{connectors} -- goal-conditioned policies that, given the current state and goal robot configuration, breaks the contact at the current configuration and remake the contact at a new configuration with the minimum disturbance to the object’s pose. For each skill, we have an associated connector that moves the robot to a state where the skill becomes applicable, similar to Mason's idea of ``funnels''~\cite{mason1985mechanics}. To train connectors, we use RL. However, the challenge is defining the right distribution of problems: if we, say, uniform-randomly generate initial state and goal configurations for connectors, we might end up training connectors on states that are irrelevant to the given PNP problem. If on the other hand, we manually design these problems, then the connector might end up facing out-of-distribution problems. Instead, we propose \texttt{Lazy Skill-RRT}, which tentatively assumes connectors exist, and teleport the robot to the next skill's applicable state. We use \texttt{Lazy Skill-RRT} to solve PNP problems, while logging the states where we teleport the robot, hence requires a connector. We then train the connector on these logged problems, which allows us to focus our connectors only on states that are likely to be encountered on a solution path. With the connectors, \texttt{Skill-RRT} can generate complete skill plans for PNP problems with diverse initial states and goal object poses.

\iffalse
To train connectors on an appropriate distribution of problems, we propose \texttt{Lazy Skill-RRT}. It tentatively assumes connectors exist, and teleports the robot to the next skill's applicable state. We use \texttt{Lazy Skill-RRT} to solve PNP problems, while logging the states where the robot is teleported and then train the connector on these logged problems. This allows connectors to focus only on states that are likely to be encountered on a solution path, rather than uniform-randomly generating connector problems, which may result in training on irrelevant states, or manually designing them, which may lead to out-of-distribution problems.

However, a key challenge with \texttt{Skill-RRT} is that the resulting state of one skill may not align with the applicable states required by the next skill. To handle such state gaps, we introduce \textit{connectors} -- goal-conditioned policies that, given the current state and goal robot configuration, breaks the contact at the current configuration and remake the contact at a new configuration with the minimum disturbance to the object’s pose. For each skill, we have an associated connector that moves the robot to a state where the skill becomes applicable, similar to Mason's idea of ``funnels''~\cite{mason1985mechanics}.

To train connectors we need to define an appropriate distribution of training problems. However, if we, say, uniform-randomly generate initial state and goal configurations for connectors, we might end up training connectors on states that are irrelevant to the given PNP problem. On the other hand, if we manually design these problems, then the connector might end up facing out-of-distribution problems.

Instead, we propose \texttt{Lazy Skill-RRT}, which tentatively assumes connectors exist, and teleport the robot to the next skill's applicable state. We use \texttt{Lazy Skill-RRT} to solve PNP problems, while logging the states where we teleport the robot, hence requires a connector. We then train the connector on these logged problems, which allows us to focus our connectors only on states that are likely to be encountered on a solution path. With the connectors, \texttt{Skill-RRT} can generate complete skill plans for PNP problems with diverse initial states and goal object poses.
\fi

While \texttt{Skill-RRT} can effectively solve long-horizon PNP problems, it requires expensive online planning, which hinders its applicability to real-world scenarios. Therefore, we use \texttt{Skill-RRT} to create solution dataset for diverse initial and goal object poses and distill it to a policy via IL to eliminate expensive online planning. Because the choice of intermediate object poses results in multi-modal trajectories, we use Diffusion Policy \cite{chi2023diffusion}. However, as already observed in the previous paper \cite{dalal2023imitating}, not all data from a planner is useful, as low-quality trajectories may degrade policy performance by leading the robot to a high-risk state. To mitigate this, we filter data by replaying the \texttt{Skill-RRT} plans with noise in simulation, and discard those whose success rate is lower than a threshold. We note that our filtering method does not require any domain knowledge, in contrast to existing approaches in prior work~\cite{dalal2023optimus}. We generate data and train all policies entirely in simulation, and zero-shot transfer to the real world.

Our framework demonstrates both effectiveness and efficiency across three contact-rich, long-horizon PNP tasks (Figure \ref{fig:CPNP_tasks}) in simulation as well as in real-world. In real-world experiments, our policy achieves \textbf{over 80\% success rates} across all domains. We also show that the distilled policy outperforms pure planner, \texttt{Skill-RRT}, PPO, an end-to-end RL algorithm, \texttt{MAPLE}~\cite{nasiriany2022augmenting}, a state-of-the-art PAMDPs-based RL algorithm, and \texttt{HLPS}~\cite{wang2024probabilistic}, a recent state-of-the-art goal-conditioned HRL algorithm, in terms of computation time and success rate.

We summarize our main contributions:
\begin{enumerate}[leftmargin=10pt, itemsep=0.3pt]
    \vspace{-0.5em}
    \item We present a novel planner, \texttt{Skill-RRT}, which extends the classical RRT algorithm into the space of skills and object goals. Unlike existing approaches, such as TAMP algorithms or PAMDPs with RL, \texttt{Skill-RRT} does not require preconditions and effects of learning-based skills or carefully designed reward functions.
    
    \item We propose \emph{connectors} to effectively bridge the state gaps that arise when sequencing independently trained skills. \texttt{Lazy Skill-RRT} identifies task-relevant state gaps that connectors should focus on, and the connectors are then trained using RL.
    
    % \item We propose \texttt{Lazy Skill-RRT}, which identifies task-relevant state gaps that arise when sequencing independently trained skills. \emph{Connectors} are then learned to bridge these gaps, thereby enabling the complete solution of PNP problems.

    \item We introduce a data filtering method that automatically selects high-quality skill plans by replaying them multiple times in simulation under domain randomization and observation noise without any domain knowledge.

    \item We demonstrate that our method achieves high success rates and reasonable computation times in both simulation and real-world experiments, while generalizing to diverse initial and goal configurations.
\end{enumerate}


==> sections/02_related_old.tex <==
\paragraph{Learning Prehensile and Non-Prehensile Skills}
% Prehensile skill
% Grasp prediction + motion planning: DexNet, contact-graspnet, Anygrasp.
% End-to-end
% Qt-opt, Joshi et al., 
There are two common approaches to learning prehensile skills.
The first approach involves incorporating grasp pose prediction and motion planning~\cite{fang2023anygrasp, mahler2017dex, sundermeyer2021contact} where the grasp prediction modules output a grasp pose given an RGB-D or point cloud observation and low-level robot joint actions are generated by a motion planner. The second approach involves training an end-to-end policy using RL~\cite{joshi2020robotic, kalashnikov2018scalable, wang2022goal}. For a more comprehensive review of prehensile skills, we encourage readers to refer to the survey by \citet{xie2023learning}. In this work, we train prehensile skills with predefined grasps using RL which can leverage GPU-parallelization to offer faster computation than a planner.

Recent studies use learning-based approaches for non-prehensile manipulation, directly mapping sensory inputs to actions to avoid the computational burden of planning, inaccuracies in hybrid dynamics models, and challenges in system identification from high-dimensional inputs. Several works \cite{ferrandis2023nonprehensile, yuan2018rearrangement, yuan2019end} focus on planar in pushing using simple cuboid objects on a tabletop, while \citet{peng2018sim} train policies for pushing pucks. \citet{zhou2023learning} train a policy for various object shapes, where the goal is to reposition the object to enable grasping, a sub-problem in PNP problems. HACMan \cite{zhou2023hacman} proposes object-centric action representations, which consist of a target point on the object point cloud and a poking direction, enabling generalization to diverse object shapes. Most of these approaches are limited to short-horizon problems, and have a restricted motion repertoire, relying primarily on planar pushing or hand-crafted primitives.

Recently, \citet{kim2023pre} have proposed an RL-based approach for non-prehensile manipulation based on a general action space that automatically discovers various skills such as toppling, sliding, pushing, pulling, etc. Moreover, this work has several features that make it suitable for PNP problems. More concretely, it decomposes the policy into a pre-contact policy, which outputs the robot configuration for contacting the object for manipulation, and a post-contact policy, which performs the manipulation. This decomposition naturally aligns with our approach to defining connectors: we train connectors to transition the robot to the pre-contact configuration, allowing skills to chain. We adopt this approach for training non-prehensile manipulation skills.

\subsection{Hierarchical Reinforcement Learning}
Hierarchical Reinforcement Learning (HRL)~\cite{sutton1999between,barto2003recent,parr1997reinforcement,dietterich2000hierarchical} aims to address long-horizon decision-making by leveraging temporally abstract actions. This abstraction improves exploration and facilitates credit assignment across extended time scales~\cite{nachum2019does}. A widely studied approach is the \textit{options framework}~\cite{sutton1999between,bacon2017option,harutyunyan2019termination}, where the agent learns options, policies that operate over multiple steps with learned termination condition $\beta$. In practice, options frequently terminate prematurely due to several structural and optimization-related factors~\cite{singh2023pear, pateria2021hierarchical, hutsebaut2022hierarchical}. First, short-term behaviors are easier to optimize during early training, as they provide denser and more reliable learning signals. In contrast, longer behaviors increase transition uncertainty and complicate credit assignment, leading to noisier gradients and slower convergence. Second, in the absence of explicit incentives to maintain temporally extended behavior, the agent is not encouraged to sustain option execution. Since most environments do not reward prolonged option usage, continuing an option beyond a few steps often wastes interaction steps without improving performance, and may even reduce overall episode efficiency due to time limits. As a result, options often collapse into primitive, one-step actions, failing to realize the intended temporal abstraction. An alternative direction is \textit{goal-conditioned HRL}~\cite{nachum2018data,zhang2022adjacency,wang2024probabilistic}, where a high-level policy proposes subgoals and a low-level policy executes them using primitive actions. While these methods have shown promising results, they often suffer from non-stationarity during training~\cite{wang2024probabilistic}, as the high-level policy must continuously adapt to the evolving behavior of the low-level policy. These methods also face structural difficulties: the subgoals proposed by the high-level policy may be unachievable by the low-level policy, or conversely, the low-level policy may be overly expressive and capable of solving arbitrary subgoals, making it difficult to discern whether successful task completion is due to effective high-level subgoal generation or robust low-level execution. This ambiguity makes assigning credit across hierarchies particularly challenging~\cite{pateria2021hierarchical}. Rather than training options or low-level policies from scratch, which is often prone to instability, inefficiency and lack of interpretability, we pre-train robotics skills using recent advances in severeal works~\cite{kalashnikov2018scalable, joshi2020robotic, kim2023pre, wang2022goal, ferrandis2023nonprehensile, yuan2018rearrangement, yuan2019end} to achieve temporal abstraction.

\subsection{Reinforcement Learning with PAMDPs}
PAMDPs~\cite{hausknecht2015deep} model decision-making with a discrete set of high-level actions, each associated with its own continuous parameters (e.g., a target pose), enabling structured and expressive action representations. This formulation has become increasingly viable due to recent advances in skill learning (Section~\ref{Related:Skills}), which provide robust and reusable low-level behaviors that generalize across a range of tasks. By reusing these low-level skills, PAMDPs reduce the complexity of training and improve stability.

Despite these advantages, PAMDPs introduce a hybrid action space, which poses challenges for standard RL algorithms. Existing methods~\cite{hausknecht2015deep, xiong2018parametrized} vary in architecture but commonly suffer from instability. This instability largely stems from the need to evaluate Q-values for parameter choices associated with unselected skills~\cite{li2021hyar}. To address this, subsequent approaches such as MAHHQN~\cite{fu2019deep} and PATRPO~\cite{wei2018hierarchical} improve stability by explicitly conditioning the parameter policy on the selected skill. However, all these methods assume that there exist states where the terminal state of one skill can directly serve as a valid initial state for the next skill. 

To address state gaps between skills, RAPS~\cite{dalal2021accelerating}, MAPLE~\cite{nasiriany2022augmenting}, and TRAPs~\cite{wang2023task} introduce a low-level primitive that directly controls single-timestep end-effector motions, supplementing a library of multi-timestep skill controllers. However, training such fine-grained motion policies is challenging, especially when long sequences of low-level actions are required to bridge large state gaps. MAPLE mitigates this through an affordance reward function that guides exploration by estimating the applicability of each skill in a given state. While effective in some cases, this approach requires designing a separate affordance for each skill, limiting scalability and generalization. In contrast, our planner \texttt{Skill-RRT} explicitly defines state gaps within the skill library, and trains additional skills, called \textit{connectors}, to bridge these gaps.

\subsection{Task and Motion Planning}
An alternative to learning-based skill sequencing is task and motion planning (TAMP). TAMP integrates discrete task planning with continuous motion planning to solve long-horizon problems by leveraging predefined skills with known preconditions and effects~\cite{garrett2021integrated}. Existing TAMP approaches are typically categorized as either sampling-based or optimization-based. Sampling-based methods~\cite{garrett2018ffrob, garrett2020pddlstream, kaelbling2011hierarchical, ren2024extended} first generate a symbolic task plan, then search for continuous parameters that satisfy geometric feasibility, or vice versa. Optimization-based approaches, such as Logic-Geometric Programming (LGP)~\cite{migimatsu2020object, toussaint2015logic, toussaint2018differentiable}, optimize symbolic plans and continuous trajectories in an interleaved manner under constraints. While TAMP has demonstrated strong performance on long-horizon problems~\cite{du2023video, kim2022representation, mendez2023embodied, vu2024coast, zhu2021hierarchical}, but, TAMP requires symbolic representations of each skill's preconditions and effects, which are often unavailable or difficult to define in PNP settings. Moreover, even when preconditions are met, skills—especially NP skills involving multiple contact-mode transitions—may fail, and successful executions often yield stochastic outcomes where the object only approximately reaches the target pose.

Similar in spirit to our approach, \citet{barry2013hierarchical} propose an RRT-based skill planner that computes a collision-free object trajectory and identifies a sequence of skills to realize it. Like our \texttt{Skill-RRT}, it extends a tree toward sampled goals using skills. However, our method differs in two key ways: we use RL-based skills that are independently trained, and we introduce connectors to bridge state gaps caused by the trained skills. More broadly, pure planners like \texttt{Skill-RRT} are computationally expensive and prone to re-planning when execution deviates from plan, particularly in contact-rich domains. We address this limitation by distilling \texttt{Skill-RRT} into a reactive policy via IL.

\subsection{Imitation Learning for Long-Horizon robot Manipulation Tasks}
Recent works have turned to IL to distill planners into reactive policies for long-horizon manipulation tasks. However, applying IL to PNP problems introduces several challenges: (1) collecting large-scale demonstration data under various initial and goal conditions, (2) ensuring the quality of demonstrations to prevent compounding errors at deployment time, and (3) handling action multi-modality caused by diverse intermediate object poses.

Collecting large-scale demonstrations remains a major bottleneck. Teleoperation-based systems~\cite{handa2020dexpilot, heo2023furniturebench, mandlekar2018roboturk, mandlekar2019scaling, stepputtis2022system} are widely used but difficult to scale, especially across diverse object configurations~\cite{brohan2022rt, xiang2019task, yang2021trail}. To overcome this, several works have proposed automated demonstration generation using simulators and planners. \citet{driess2021learning} generate TAMP datasets by solving plans with Logic-Geometric Programming (LGP) and executing them in the Bullet simulator via Model Predictive Control (MPC) to train low-level policies.
\citet{mcdonald2022guided} build TAMP datasets by using FastForward for task planning and refining motion trajectories in simulators, including 2D pick-place, RoboSuite, and RoboDesk, to train hierarchical policies that imitate both task and motion planning.
OPTIMUS~\cite{dalal2023imitating} generates trajectories using PDDLStream~\cite{garrett2020pddlstream}, combining symbolic planning with grasping, placing, and inverse kinematics samplers to train low-level policies. We take a similar approach but use \texttt{Skill-RRT}, a skill-level planner specifically designed for PNP problems. Unlike symbolic task planners, \texttt{Skill-RRT} plans directly over parameterized skills and connectors, ensuring feasibility across skill transitions.

Even with abundant data, training with low-quality demonstrations can lead to failure and out-of-distribution states during policy deployment~\cite{mandlekar2022matters}. OPTIMUS addresses this by applying a containment constraint, filtering out trajectories where the end-effector exits a predefined workspace. While effective, such heuristics are domain-specific, often require human knowledge or manual intervention, and do not generalize well to diverse manipulation tasks. Instead, we evaluate the robustness of each plan by replaying it under stochastic disturbances in a simulator, keeping only plans that succeed under noise. This allows us to construct a clean, high-quality IL dataset without relying on human intervention.

To address action multi-modality, prior works have proposed various architectural strategies. \citet{lee2024behavior} and \citet{shafiullah2022behavior} combine discrete action classifiers with continuous refiners to distinguish and fine-tune different behavioral modes. ACT~\cite{Zhao-RSS-23} employs conditional variational autoencoders (CVAEs) within a transformer to generate fixed-length action sequences. OPTIMUS~\cite{dalal2023imitating} represents diverse interaction modes using a Gaussian Mixture Model, capturing variations in grasp, placement, and trajectory. Diffusion Policy~\cite{chi2023diffusion} introduces diffusion models for imitating action distributions and achieves strong real-world results. Building on these insights, we also adopt Diffusion Policy, as our skill planner generates diverse intermediate subgoal object poses even for the same problem instance (i.e., identical \( s_0 \) and \( q^g_\text{obj} \)), resulting in multi-modal action distributions. Diffusion models are well-suited to capture such diversity, making them an appropriate choice for our setting.

==> sections/02_related_short.tex <==
\subsection{Learning Prehensile and Non-Prehensile Skills}\label{Related:Skills}
Prehensile skill learning typically follows two approaches. One combines grasp pose prediction with motion planning~\cite{fang2023anygrasp, mahler2017dex, sundermeyer2021contact}, where grasp poses are predicted from RGB-D or point cloud inputs and executed via planners. The other trains end-to-end RL policies to grasp diverse objects through trial and error~\cite{joshi2020robotic, kalashnikov2018scalable, wang2022goal}. For a broader review, see~\citet{xie2023learning}. In this work, we use predefined grasp poses and train RL-based prehensile skills with GPU-parallelization for faster computation than planning.

Non-prehensile manipulation has also been studied through learned policies that avoid planning and model inaccuracies. Prior works focus on planar pushing~\cite{ferrandis2023nonprehensile, yuan2018rearrangement, yuan2019end}, object repositioning~\cite{zhou2023learning}, and object-centric poking~\cite{zhou2023hacman}. However, these methods often operate in short horizons with limited motion diversity.

\citet{kim2023pre} propose an RL-based approach using a general action space that discovers diverse non-prehensile skills like toppling, pushing, and pulling. Their method decomposes the policy into pre-contact and post-contact phases, aligning with our connector-based chaining: we train connectors to reach the pre-contact configuration of each skill, enabling sequential skill composition. We adopt this framework for skill training in our work.


\subsection{Hierarchical Reinforcement Learning}
Hierarchical Reinforcement Learning (HRL)~\cite{sutton1999between,barto2003recent,parr1997reinforcement,dietterich2000hierarchical} aims to address long-horizon decision-making by leveraging temporally abstract actions. This abstraction improves exploration and facilitates credit assignment across extended time scales~\cite{nachum2019does}. A widely studied approach is the \textit{options framework}~\cite{sutton1999between,bacon2017option,harutyunyan2019termination}, where the agent learns macro-actions—policies that operate over multiple steps with learned termination. However, in practice, options often degenerate into primitive actions or terminate prematurely unless regularized properly~\cite{singh2023pear}, thereby limiting the intended benefits of temporal abstraction. An alternative direction is \textit{goal-conditioned HRL}~\cite{nachum2018data,zhang2022adjacency,wang2024probabilistic}, where a high-level policy proposes subgoals and a low-level policy executes them using primitive actions. While these methods have shown promising results, they often suffer from non-stationarity during training~\cite{wang2024probabilistic}, as the high-level policy must continuously adapt to the evolving behavior of the low-level policy. These methods also face structural difficulties: the subgoals proposed by the high-level policy may be unachievable by the low-level controller, and assigning credit across hierarchies remains a key challenge~\cite{pateria2021hierarchical}. Rather than training macro-actions or low-level policies from scratch, which is often prone to instability and inefficiency, we leverage recent advances in robotic skills~\cite{kalashnikov2018scalable, joshi2020robotic, kim2023pre, wang2022goal, ferrandis2023nonprehensile, yuan2018rearrangement, yuan2019end} as structured low-level controllers to achieve temporal abstraction in a more scalable and reusable way.

\subsection{Reinforcement Learning with PAMDPs}
PAMDPs~\cite{hausknecht2015deep} provide a modular alternative to HRL by decoupling high-level planning from fixed low-level controllers. This separation, enabled by recent advances in skill learning (Section~\ref{Related:Skills}), improves training stability and scalability by reusing robust, task-agnostic low-level skills. However, PAMDPs introduce a hybrid action space, combining discrete skill selection with continuous parameterization, which challenges standard RL algorithms. Methods like PADDPG~\cite{hausknecht2015deep} and PDQN~\cite{xiong2018parametrized} address this with joint or hierarchical architectures, but suffer from instability due to Q-value interference from unselected skills~\cite{li2021hyar}. Later approaches such as MAHHQN~\cite{fu2019deep} and PATRPO~\cite{wei2018hierarchical} improve stability by conditioning parameters on the chosen skill. Nonetheless, they assume that the terminal state of one skill can directly serve as a valid initial state for the next. RAPS~\cite{dalal2021accelerating}, MAPLE~\cite{nasiriany2022augmenting}, and TRAPs~\cite{wang2023task} use single-step end-effector primitives to bridge skill gaps, but training such low-level controllers is challenging, especially for long transitions. MAPLE introduces affordance-based rewards to guide skill selection, though these require manual design for each skill. In contrast, \texttt{Skill-RRT} explicitly defines state gaps and learns \textit{connectors} to bridge them, enabling robust composition of independently acquired skills.

\subsection{Task and Motion Planning}
An alternative to learning-based skill sequencing is to explicitly plan over skills using symbolic task and motion planning (TAMP)~\cite{garrett2021integrated}. TAMP combines symbolic planning with geometric reasoning, using either sampling-based~\cite{garrett2018ffrob, garrett2020pddlstream, kaelbling2011hierarchical, ren2024extended} or optimization-based approaches such as Logic-Geometric Programming (LGP)~\cite{migimatsu2020object, toussaint2015logic, toussaint2018differentiable}. While effective~\cite{du2023video, kim2022representation, mendez2023embodied, vu2024coast, zhu2021hierarchical}, these methods require explicit preconditions and effects for each skill, which are often unavailable in PNP settings.

\citet{barry2013hierarchical} propose an RRT-based skill planner that extends a tree using skills to follow an object trajectory, similar to our \texttt{Skill-RRT}. However, we use independently acquired RL-based skills and train connectors to bridge infeasible transitions. More broadly, planners like \texttt{Skill-RRT} are costly and sensitive to execution errors in contact-rich tasks. We address this by distilling \texttt{Skill-RRT} into a reactive policy via IL.

\subsection{Imitation Learning for Robotics}
IL is commonly used to distill planners into reactive policies for long-horizon tasks. In PNP settings, IL faces three main challenges: (1) collecting diverse demonstrations, (2) ensuring demonstration quality, and (3) modeling action multi-modality.

For data collection, teleoperation-based methods~\cite{handa2020dexpilot, heo2023furniturebench, mandlekar2018roboturk, mandlekar2019scaling, stepputtis2022system} are widely used but hard to scale~\cite{brohan2022rt, xiang2019task, yang2021trail}. Alternatives leverage simulation and planning. \citet{driess2021learning} use LGP with MPC; \citet{mcdonald2022guided} combine FastForward with motion planning; OPTIMUS~\cite{dalal2023imitating} uses PDDLStream~\cite{garrett2020pddlstream} with grasp and IK samplers. We follow this direction but employ \texttt{Skill-RRT}, which plans directly over parameterized skills and connectors for PNP-specific transitions.

Demonstration quality is also critical, as low-quality data leads to OOD failures~\cite{mandlekar2022matters}. OPTIMUS filters trajectories via containment constraints, but such heuristics require domain knowledge and limit generalization. In contrast, we filter by replaying plans under noise and keeping only those robust to disturbance, avoiding manual intervention.

To model action multi-modality, prior works use discrete mode prediction~\cite{lee2024behavior, shafiullah2022behavior}, CVAEs~\cite{Zhao-RSS-23}, or GMMs~\cite{dalal2023imitating}. Diffusion Policy~\cite{chi2023diffusion} leverages diffusion models to sample diverse behaviors. We adopt this approach to capture the variability of subgoal-induced trajectories in PNP tasks.


==> sections/03_method_old.tex <==
% how constructed methodology
% \input{tables/notations/state}
% \input{tables/notations/skill}
% \input{tables/notations/skill-rrt}
% \input{tables/notations/connector}
% \input{tables/notations/IL}
\begin{figure*}[t] % Force the figure at the top of the page
\centering
\vspace{-5mm}
\resizebox{\textwidth}{!}{
    \includegraphics{figures/cpnp_overview_v7.png}
}
% \caption{Overview of our method: (a) A skill library $\mathcal{O}$ that consists of $n$ number of non-prehensile (NP) and $m$ number of prehensile (P) skills are given. (b) We first train connector skills. To do this, we use \texttt{Abstract Skill-RRT} to collect pairs of states that the connector needs to connect, based on the preconditions and effects of the skills in $\mathcal{O}$, and the connectors are trained using reinforcement learning (RL). (c) We then generate data for imitation learning by running \texttt{Skill-RRT} with the skills in $\mathcal{O}$ and connector skill. Given an initial node $q_{\text{init}}$ (red circle) and a goal object pose $q^{\text{obj}}_{\text{goal}}$ (green circle), we generate a skill plan $\tau_{\text{skill}}$, which includes a sequence of skills (blue lines), connectors (yellow lines), and their associated subgoals (black circle). (d) We filter out low-quality data by replaying each skill plan N times, and filtering skill plans with low replay success rate based on a pre-defined threshold $\theta$. The filtered trajectories are used to train diffusion policy. The final diffusion policy is deployed in the real world in a zero-shot manner. }\label{fig:CPNP_overview} % Place the label after the caption
\caption{Overview of our method: (a) Examples of given skills in the bookshelf domain~(Figure~\ref{fig:CPNP_tasks}, row 2). $K_\text{P}$ is a prehensile skill, $K_{\text{NP}_1}$ is a toppling skill that topples a book, and $K_{\text{NP}_n}$ is a pushing skill that pushes an object at a bottom shelf. (b) We first use \texttt{Lazy Skill-RRT} to collect a set of $(v.s, v_{\text{connect}}.s, K)$ triplets which defines the connections the connectors need to make, and $v$ denotes a node of RRT. The middle of (b) shows an example where the connector has to move the gripper from the end of the prehensile skill's state, $v.s$, to the beginning of the pushing skill, $v_{\text{connect}}.s$. We use RL to train connectors. (c) \texttt{Skill-RRT} is run with the trained connectors $\mathcal{C}$ and the set of skills $\mathcal{K}$ to generate a skill plan $\tau_{\text{skill}}$. Starting from the initial node $s_{0}$ (red circle) and the goal object pose $q_{\text{obj}}^{g}$ (green circle), the skill plan consists of a sequence of skills, connectors, and their associated desired object poses, or desired robot configuration (black circles). (d) We use IL to distill skill plans into a single policy. To filter data, we replay each skill plan $N$ times, and those with a replay success rate below a predefined threshold $m$ are filtered out. The remaining high-quality trajectories are used to train a diffusion policy, which is deployed in the real world in a zero-shot manner.}\label{fig:CPNP_overview}
\end{figure*}

\subsection{PNP manipulation problem formulation}\label{method:PF}

% Description of Notation
We denote the state space as $S$, the action space as $A$. A state $s \in S$ includes object pose and velocity, robot joint positions, and velocities, denoted $\qobj, \vobj, \qrobot$ and $\vrobot$ respectively. An action $a \in A$ consists of the target end-effector pose, the gain and damping values for a low-level differential inverse kinematics (IK) controller, and the target gripper width enabling forceful action for NP skills. We represent the space of stable and relevant object configurations as $\Qobj \subset SE(3)$. This space includes only regions represented as $SE(2)$ where the object can occupy, determined by environmental constraints like the presence of shelves. For example, in the bookshelf domain, a book can be placed only between other books on the upper shelf or laid flat on a box on the lower shelf.

% We denote the state space as $S$, action space as $A$, and space of stable and relevant object configurations as $\Qobj \subset SE(3)$, which only includes regions where the object can occupy, determined by environmental constraints like the presence of shelves. A state $s \in S$ includes object pose and velocity, robot joint positions, and velocities, denoted $\qobj, \vobj, \qrobot$ and $\vrobot$ respectively. An action $a \in  A$ consists of the target end-effector pose, the gain and damping values for a low-level differential inverse kinematics (IK) controller, and the target gripper width.


% Emphasize that skills are given
We assume we are given a set of manipulation skills, $\skillset=\{\pskill,K_{\text{NP}_1},\cdots,K_{\text{NP}_n}\}$, one of which is prehensile (P) and the rest are non-prehensile (NP) skills. For instance, in the bookshelf domain, we have a \textit{topple} and \textit{push} NP skills, and one P skill for pick-and-placing the book to a target object state. Each skill $K$ is a tuple of two functions, $K =\{ \applicabilitychecker, \pi\}$, where $\pi: S \times \Qobj \rightarrow A$ is a goal-conditioned policy that maps a state $s$ and a desired object pose $\qobj$ to an action\footnote{More accurately, we use quantities derived from $s$. See Appendix~\ref{Appendix:NP_Skill},~\ref{Appendix:P_Skill} and~\ref{Appendix:Connector}}. We train our skills using RL, using the same policy computation structure from~\cite{kim2023pre}, where our policy $\pi$ consists of $\pipre$ and $\pipost$\footnote{$\pipre$ uses a different action space to ensure contact. See Appendix~\ref{Appendix:NP_Skill} and~\ref{Appendix:P_Skill}.}. $\pipre$ is a \emph{pre-contact} policy that predicts the robot configuration prior to executing the \emph{post-contact} policy that actually manipulates the object. For instance, for our prehensile skill, $\pipre$ puts the robot at a pre-grasp configuration, and $\pipost$ places the object. 

\iffalse
% Justification for why the region is necessary for the skills 
We denote the space of stable and relevant object configurations as $\Qobj \subset SE(3)$, which only includes regions where the object can occupy, determined by environmental constraints like the presence of shelves. We associate each skill with a region where it is applicable, defined as a subset of $\Qobj$ in which the skill can reliably operate. This concept follows prior work on both prehensile skills in TAMP~\cite{garrett2021integrated} and non-prehensile skills~\cite{kim2023pre}, where the space of valid initial and goal object poses is known. For example, a sliding skill moves a card from one pose to another while the card remains flat on the table, either face-up or face-down. This is essential because sampling feasible object poses directly from the full $SE(3)$ space is often intractable.

% To use independently defined skills in a unified way, we associate each skill with a region where it is applicable, defined by the object configurations in which the skill can reliably operate. This idea is motivated by prior work in both prehensile~\cite{nasiriany2022augmenting} and non-prehensile~\cite{kim2023pre} manipulation, where problems are commonly formulated as moving an object from an initial pose to a goal pose. For example, a sliding skill moves a card from one pose to another while the card remains flat on the table, either face-up or face-down. Prehensile skills like placing are often parameterized by the end-effector pose, but after grasping, the object pose is effectively determined by the end-effector motion. As such, describing each skill by the set of object poses it can move the object from and to is equivalent to defining a region, allowing both prehensile and non-prehensile skills for a unified formulation.

% We then define $\Qobj$ as the union of the applicable regions for all given skills. This construction ensures that $\Qobj$ captures exactly the subset of object configurations that are reachable using the available skill library. Configurations outside of $\Qobj$ are excluded from planning, as no skill can transition the object into or out of those states.

% Description of Skill
Each skill $K$ is a tuple of two functions, $K =\{ \applicabilitychecker, \pi\}$, where $\pi: S \times \Qobj \rightarrow A$ is a goal-conditioned policy that maps a state $s$ and a desired object pose $\qobj$ to an action\footnote{More accurately, instead of using $s$ directly, we use quantities derived from $s$. See Appendix~\ref{Appendix:NP_Skill},~\ref{Appendix:P_Skill} and~\ref{Appendix:Connector}}. We train our skills using RL, using the same policy computation structure from~\cite{kim2023pre}, where our policy $\pi$ consists of $\pipre$ and $\pipost$\footnote{$\pipre$ uses a different action space to ensure contact. See Appendix~\ref{Appendix:NP_Skill} and~\ref{Appendix:P_Skill}.}. $\pipre$ is a \emph{pre-contact} policy that predicts the robot configuration prior to executing the \emph{post-contact} policy that actually manipulates the object. For instance, for our prehensile skill, $\pipre$ puts the robot at a pre-grasp configuration, and $\pipost$ places the object. 
\fi

One well-known problem  when planning with parameterized manipulation skills is that if you sample the object pose $\qobj$ from the full $SE(3)$ space, the probability of sampling a stable pose is zero, and planning becomes intractable~\cite{garrett2021integrated}. Therefore, following the prior work~\cite{garrett2021integrated}, we associate each distinct region of stable poses with a NP skill while the region for a P skill is defined as the union of these regions, which corresponds to $\Qobj$. For example, in the bookshelf domain, the upper shelf is associated with topple or push skills, the lower shelf is associated with the push skill, and the P skill enables moving the book between these regions.

\iffalse
Each NP skill is associated with a distinct region where it is applicable, defined as a subset of $\Qobj$ in which the NP skill can reliably operate. The region of P skill is defined as the union of the regions for all NP skills, which corresponds to $\Qobj$. For example, in the bookshelf domain, the topple skill moves a book within a crowded upper shelf, the push skill operates within a lower shelf, and the P skill moves the book in both regions. This concept follows prior work on both P skills in TAMP~\cite{garrett2021integrated} and NP skills~\cite{kim2023pre}, where the space of valid initial and goal object poses is known. The notion of regions enables sampling of feasible object poses within a reasonable time, rather than randomly sampling from the full $SE(3)$ space, which is often intractable for identifying feasible object poses.
\fi

% Description of applicability checker
The function $\applicabilitychecker:S \times \Qobj \rightarrow \{0,1\}$ is an applicability checker that tests whether it is possible to execute the skill policy in $s$ with $\qobj \in \Qobj$ as its goal. This could be an IK solver that checks the existence of a feasible grasp for both the current and target object poses for a prehensile skill, or a simple check for whether the desired and the current object pose belong to the same region for an NP skill. Note that $\phi$ only checks whether skill \textit{can} be applied in the current state, and not whether the skill would succeed. Lastly, we assume we have a simulator $\fsim$ that takes in state $s$ and $\pi(\cdot;\qobj)$, a policy conditioned on desired object pose $\qobj$, and simulates the policy for $N_{sim}$ number of time steps, and returns the next state, $\fsim: S \times \Pi \rightarrow S$ where $\Pi$ is the set of policies of skills defined in $\skillset$. 

Given a pair of an initial state $s_0 \in S$ and the ultimate goal object pose $\qobj^g \in \Qobj$, the objective of a PNP problem is to find a sequence of actions for achieving $\qobj^g$. Because our policies output actions, this problem reduces to finding the sequence of skills and associated intermediate object poses, that we call a \textit{skill plan}, $\skillplan = \{\pi^{(t)},q^{(t)}\}_{t=1}^{T}$, such that when we simulate the sequence of $T$ policies from $s_0$, the resulting state would have $\qobj^g$ as its object pose.

At a high-level, our method uses \texttt{Skill-RRT} to collect data, and then distill it to a policy using IL. But to find the trajectories using \skillrrt, we first need connectors, and to do that, we need \lazyskillrrt~to collect relevant skills and states for which to train connectors. See Figure~\ref{fig:CPNP_overview} for the overview. We first introduce \texttt{Skill-RRT}, from which you can define \lazyskillrrt.

\subsection{Skill-RRT}

% Emphasize the skill is independently acquired, and the region won't hint the solution
% However, this planning problem is nontrivial. Independently acquired skills do not suggest how to be composed into a complete plan. Since each skill is defined in isolation and operates within its own region, the output of one skill may not satisfy the conditions required by another. As a result, additional transitions are often needed to bridge between skills. To address this, we propose \texttt{Lazy Skill-RRT}, a planning method that discovers where such transitions are needed. These transitions are then handled by connector policies, which we describe in Section~\ref{method:train_connector}.


\begin{wrapfigure}{r}{0.55\textwidth}
\vspace{-2em}
\begin{minipage}{0.55\textwidth}
\begin{algorithm}[H]
\small
\caption{\skillrrt($s_0, \qobj^g, \skillset, \connectorskillset,\Qobj$)}
\label{algo:skillrrtbackbone}
\begin{algorithmic}[1]
\State $T=\emptyset$   
\State $v_{0} \gets \{(\emptyset, \emptyset), s_0\}$ 
\State $T$.\texttt{AddNode}($parent=\emptyset, child=v_{0}$)
\For{$i = 1$ \textbf{to} $N_{\text{max}}$}
    \State ${K}, \qobj \gets $\hyperref[algo:UnifSmplSkillAndSubgoal]{\texttt{UnifSmplSkillAndSubgoal}}($\skillset,\Qobj$)
    \State ${v}_{\text{near}} \gets$ \hyperref[algo:GetFeasibleNearestNode]{\texttt{GetApplicableNearestNode}}($T, K, \qobj$)

    \If{$v_\text{near}$ is $\emptyset$} 
        \State \textbf{continue}
    \EndIf
    \State \hyperref[algo:extend]{\texttt{Extend}}$\big(T, K, v_{\text{near}}, \qobj, \connectorskillset\big)$
    \If{\texttt{Near}($\qobj^g,T$)}
        \State \textbf{Return} \texttt{Retrace}($\qobj^g, T$)
    \EndIf
\EndFor
\State \textbf{Return} None
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-1em}
\end{wrapfigure}

Algorithm~\ref{algo:skillrrtbackbone} provides the pseudocode for \skillrrt. The algorithm takes as input an initial state $s_0$, goal object configuration $\qobjg$, set of skills $\skillset$, set of connectors $\connectorskillset$, and object regions $\Qobj$. As we will soon explain, setting $\connectorskillset$ to an empty set makes it \lazyskillrrt.

The algorithm begins by initiating the tree, $T$, with an empty set, defining the root node, and adding it to the tree (L1-3). A node $v$ consists of a state $s$ and a pair of a skill policy $\pi$ and its desired object pose $\qobj$ that have been applied to the parent state to achieve the current state. For the root node, the policy and pose are set to an empty set (L2). We then begin the main for-loop. We first uniform-randomly sample a skill $K$ and the desired object pose for the skill, $\qobj$, using the function \hyperref[algo:UnifSmplSkillAndSubgoal]{\texttt{UnifSmplSkillAndSubgoal}} (L5), and then compute the nearest node from the tree among the nodes where $K$ can be applied (L6). Specifically, \hyperref[algo:GetFeasibleNearestNode]{\texttt{GetApplicableNearestNode}} function returns the nearest node $v$ where $K.\phi(v.s, \qobj)$ is true, and an empty set if no such node exists. If the function returns an empty set, we discard the sample, and move to the next iteration (L7-8). Otherwise, we use \hyperref[algo:extend]{\texttt{Extend}} function with $v_{near}$ (L9). Lastly, at every iteration, we check if $\qobjg$ is close enough to any of the nodes in the tree, and if it is, return the path by calling the \texttt{Retrace} function that computes a sequence of $v$ from root node to that node (L10-11). If no such node can be found after $N_{max}$ number of iterations, we return None (L12).

\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-2em}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\small
\caption{\texttt{Extend}($T, \skill, \node, \qobj', \connectorskillset$)}
\label{algo:extend}
\begin{algorithmic}[1]
\State $\qrobot' \gets \skill.\pipre(\node.s.\qobj;\qobj')$
\State $\connectingnode \gets \hyperref[algo:computeconnectingnode]{\texttt{ComputeConnectingNode}}(\qrobot', \skill,\connectorskillset, \node)$
\State $s' \gets \fsim(\connectingnode.s, \skill.\pipost(\connectingnode.s;\qobj'))$
\If{$\hyperref[algo:Failed]{\texttt{Failed}}(s', \qobj')$}
\State \Return
\EndIf
\State $v' \gets (\skill.\pipost, \qobj',s')$
\State $T.\texttt{Add}(parent=\node, child=\connectingnode)$
\State $T.\texttt{Add}(parent=\connectingnode, child=\node')$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-1.5em}
\end{wrapfigure}

Algorithm~\ref{algo:extend} shows the $\texttt{Extend}$ function. The function takes in the tree $T$, skill to be simulated $K$, node $v$ that we will use $K$ from, desired object pose we will extend to, $\qobj'$, and set of connectors $\connectorskillset$. The algorithm begins by computing a pre-contact robot configuration for $K$, $\qrobot'$, using $K$'s pre-contact policy at state $v.s$ with $\qobj'$ as a goal (L1). It then creates a connecting node, using $\texttt{computeconnectingnode}$ shown in Algorithm~\ref{algo:computeconnectingnode} (L2-3).

Algorithm~\ref{algo:computeconnectingnode} shows the $\texttt{ComputeConnectingNode}$ function. The function takes as input the target robot joint configuration \( q_r' \), the skill \( K \) to be simulated, the connector set \( \mathcal{C} \) which includes connector policies, and the node \( v \) from which the connector policy or teleportation is applied.
The algorithm begins by checking if $\connectorskillset$ is empty, in which case this will instantiate \lazyskillrrt (L1). In this case, we create a connecting node $\connectingnode$ with empty skill and object pose, with the same state as $v$, except the robot joint configuration is teleported to $\qrobot'$ (L2-4). Otherwise, we retrieve the connector $\pi_C$ for the given skill $K$ (L6), simulate it from $v.s$ with pre-contact configuration $\qrobot'$ as a goal (L7), and create $\connectingnode$ using $\pi_C$, $\qrobot'$, and the resulting state $s'$ (L8).

\begin{wrapfigure}{r}{0.53\textwidth}
\vspace{-2em}
\begin{minipage}{0.53\textwidth}
\begin{algorithm}[H]
\small
\caption{\texttt{ComputeConnectingNode}($\qrobot', \skill, \connectorskillset, \node$)}
\label{algo:computeconnectingnode}
\begin{algorithmic}[1]
\State IsLazy $\gets \connectorskillset == \emptyset$
\If{IsLazy}
\State $\connectingnode \gets (\emptyset, \emptyset, \node.s)$
\State $\connectingnode.s.\qrobot \gets \qrobot'$ \Comment{Teleport the $q_r$ to $q_r'$}
\Else
\State $\pi_C \gets \texttt{GetConnectorForSkill}(\connectorskillset,\skill) $
\State $s' \gets \fsim(\node.s, \pi_C(v.s;\qrobot'))$
\State $\connectingnode \gets (\pi_C,\qrobot', s')$
\EndIf
\Return $\connectingnode$
\end{algorithmic}
\end{algorithm}
\end{minipage}
\vspace{-1.5em}
\end{wrapfigure} 

We then return the connecting node $\connectingnode$ to the \texttt{Extend} function in Algorithm~\ref{algo:extend} (L2-3). From the connecting node's state, $\connectingnode.s$, we simulate the post-contact policy $\pipost$  with $\qobj'$ as its goal (L3). If the skill fails to achieve $\qobj'$, then we return without modifying the tree (L4-5). Otherwise, we create a new node $\node'$ with the resulting state $s'$, simulated policy $\skill.\pipost$, and the desired object pose $\qobj'$ (L6). We add $\connectingnode$ with its parent as $\node$, and $\node'$ with $\connectingnode$ as its parent (L7-8).

%For \lazyskillrrt, we pass in empty set for $\connectorskillset$ to \skillrrt, 
%We use this backbone to define \lazyskillrrt~that teleports the robot to the pre-contact configuration in simulation. Algorithm~\ref{algo:lazyextend} describes the algorithm. The algorithm takes as input the tree $T$, skill that will be simulated, $K$, the node to extend from, $v$, and the target object pose for the skill, $\qobj'$. The algorithm begins by computing the pre-contact robot configuration for the skill, $\qrobot'$ (L1). It then creates the node that \textit{would have} resulted \emph{if} we had executed a connector policy from $v$, $\connectingnode$, which practically have the same state as $\node$ except the robot configuration at $\qrobot'$ and $K.\pipre$ as its policy (L2-3). We then simulate the post-contact policy from the state of $\connectingnode$ with $\qobj'$ as its goal to get the resulting state $s'$, and check if the skill has achieved $\qobj'$. If not, we return without modifying the tree (L4-6). Otherwise, we create a new node $\node'$ with the resulting state $s'$, simulated policy $\skill.\pipost$, and the target object pose (L7). We add $\connectingnode$ with its parent as $\node$, and also $\node'$ with $\connectingnode$ as its parent. \lazyskillrrt~is defined as an instantiation of \skillrrtbackbone~with \texttt{LazyExtend} as the extend function.

This gives only a high-level description of some of the subroutines such as \hyperref[algo:UnifSmplSkillAndSubgoal]{\texttt{UnifSmplSkillAndSubgoal}}, \hyperref[algo:GetFeasibleNearestNode]{\texttt{GetApplicableNearestNode}} or \hyperref[algo:Failed]{\texttt{Failed}}~for brevity and clarity. Their detailed pseudocodes and GPU-parallelized version used in our experiments are in Appendix~\ref{Appendix:Skill-RRT Details}.

\subsection{Training the connectors}\label{method:train_connector}
% we need skills for filling the gap.
% the gap is ~~~.
% we 저러한 gap을 매우기 위하여 추가적인 connector 라는 skill을 학습하기로 결정했다. 이는 RL을 통한 policy가 object 및 env와 다양한 contact 이 있는 상황에서도 잘 작동하기 때문.
% independently train skill library state gap 그리고, motion planner

% identify gap
% The state gap caused by independently trained skills is  reveal missing actions caused by teleportation of robot configurations in Algorithm~\ref{algo:computeconnectingnode} (L3-4). We first generate PNP problems with initial and goal pairs \( (s_0, \qobjg) \), and run Algorithm~\ref{algo:skillrrtbackbone} with \( \connectorskillset = \emptyset \). From the resulting solution, we identify connecting nodes that represent missing transitions between consecutive skills. For each $\connectingnode$, we collect a training triplet \( (\node.s, \connectingnode.s, K) \), where \( \node \) is its parent and \( K \) is the skill used to reach the next node (child of $\connectingnode$). Here, \( \node.s \) serves as the initial state and \( \connectingnode.s.q_r \) as the goal for training the connector policy \( \pi_C \).

% 그 문제를 풀기 위해 무조건 수반되어야 하는 state gap
% \texttt{Lazy Skill-RRT} identifies likely state gaps that may hinder successful object manipulation when chaining skills to solve the task, enabling targeted resolution only for transitions that are actually required. It generates skill plans by running Algorithm~\ref{algo:skillrrtbackbone} with an independently trained skill library \( \mathcal{K} \) and an empty connector set \( \connectorskillset = \emptyset \). These gaps result from the teleportation of robot configurations in Algorithm~\ref{algo:computeconnectingnode} (Lines 3–4), and are represented by connecting nodes that mark the gaps between consecutive skills. For each connecting node $\connectingnode$, we extract a triplet \( (\node.s, \connectingnode.s, K) \), where \( \node \) is its parent and \( K \) is the skill applied from $\connectingnode$ to its child. In this triplet, \( \node.s \) serves as the initial state and \( \connectingnode.s.q_r \) as the goal, forming a concrete instance of a state gap.

% To obtain connectors for each skills $\connectorskillset$, we collect problems using \lazyskillrrt{} by first creating a PNP problem that consists of a pair $(s_0,\qobjg)$, and then running Algorithm~\ref{algo:skillrrtbackbone} with $\connectorskillset=\emptyset$. This will return a solution node sequence, some of which will be $\connectingnode$. We then collect a set of $(\node.s,\connectingnode.s,K)$ triplet from the node sequence, where $\node$ is the parent of $\connectingnode$, and $K$ is the skill that was used from $\connectingnode$ to get its child node.

% We train a connector policy $\pi_C$ for each skill $K$ using RL. A naïve implementation of connectors would be to use a collision‑free motion planner (MP) to reposition the gripper, yet in practice this strategy fails for several reasons. For example, control errors (i.e., the robot’s inability to exactly follow the planned path) often disturb the card and can even cause it to fall off the table. The detailed discussion of these failure cases is provided in Appendix~\ref{Appendix:Connector_vs_MP}. In contrast, connectors trained via RL offer key advantages: they account for contact-induced object dynamics and remain effective in confined spaces where MP often fail. Accordingly, we train each connector policy using PPO~\cite{schulman2017proximal}, and the detailed MDP formulation is provided in Appendix~\ref{Appendix:Connector}.

To train a set of connectors $\connectorskillset$, we collect problems using \lazyskillrrt{} by first creating a PNP problem that consists of a pair $(s_0,\qobjg)$, and then running Algorithm~\ref{algo:skill-rrt} with $\connectorskillset=\emptyset$. This will return a solution node sequence, some of which will be $\connectingnode$. We then collect a set of $(\node.s,\connectingnode.s,K)$ triplet from the node sequence, where $\node$ is the parent of $\connectingnode$, and $K$ is the skill that was used from $\connectingnode$ to get its child node.

% There is something odd about the definition of K above.
% Why is this a skill used from v_connect? Because we need to know what skill came after the connecting node, because we need the skill associated with the connector that got us to v_connect

We then train a connector $\pi_C$ for each $K$, whose goal is to go from $\node.s$ to the connecting node's robot configuration $\connectingnode.s.\qrobot$, using PPO~\cite{schulman2017proximal}, with minimum disturbance to the object pose in $\node.s$. This is a goal conditioned policy that maps a state to an action, $\pi_C(\cdot;\qrobot): S \rightarrow A$. The reward consists of four main components, $r_{\text{connector}} = r_{\text{ee}} + r_{\text{tip}} + r_{\text{obj-move}} + r_{\text{success}}$,
where $r_{\text{ee}}$ and $r_{\text{tip}}$ are dense rewards based on the distances between the current and target end-effector poses and gripper tip positions, respectively. $r_{\text{obj-move}}$ penalizes an action if it changes the object pose from previous object pose, and $r_{\text{success}}$ gives a large success reward for achieving the target end-effector pose and gripper width. More details about the implementation of these reward terms can be found in Appendix~\ref{Appendix:Connector}.


\subsection{Distilling \skillrrt~to a policy for real-world deployment}\label{method:IL}
We adopt imitation learning (IL) to address the inefficiency of planning with \texttt{Skill-RRT}, which limits its practicality for real-world deployment. Our goal is to train an IL policy, $\pi_\text{IL}: S_{\text{IL}}\times Q_\text{obj} \rightarrow A$, that enables faster inference while generalizing to diverse initial states and goals. Unlike human demonstrations, which are expensive to collect across a wide variety of initial states and goals, we use \texttt{Skill-RRT} to solve multiple PNP problems in simulation, generate state-action trajectories, and distill them into a single policy using IL.

Training \( \pi_\text{IL} \) requires two key design choices: (1) selecting high-quality skill plans to use for IL training, and (2) choosing the appropriate policy architecture that accounts for the characteristics of our data.
For (1), we introduce a skill plan quality evaluation method for filtering training data. Each plan is replayed $N$ times in parallel with noise injected into observations and joint torque, and randomized physical parameters such as friction and mass. Plans with a success rate above a threshold $m$, i.e., $\frac{N_{success}}{N} > m$, are retained. This process ensures that the dataset remains robust to perception and modeling errors and prioritize solutions that are more likely to reach the goal despite these uncertainties. For example, in the Card Flip domain, placing the card at the far end of the table may technically succeed, but such plans will frequently fail even with small perception or dynamics errors. Our filtering mechanism identifies and removes such unreliable plans by replaying them multiple times under noise. Details of evaluation process are provided in Appendix~\ref{Appendix:data_qual}. For (2), even for the same problem (i.e., the same \( s_0 \) and \( q^g_\text{obj} \)), demonstrations will exhibit different intermediate subgoals, resulting in diverse state and action distributions. Hence, we adopt Diffusion Policy~\cite{chi2023diffusion} to handle the multi-modality present in our data. To enable faster inference in Diffusion Policy, we use a U-Net~\cite{ronneberger2015u} as the policy backbone and remove both action chunking and state history. As a result, the policy can generate actions at 75 Hz on an NVIDIA RTX 4090 GPU, enabling faster real-time inference. The details about $\pi_\text{IL}$ training, such as slightly different state space from the skill's, are provided in Appendix~\ref{Appendix:imitation_learning}.

==> sections/04_experiment_old.tex <==
\subsection{Simulation results}
We evaluate our method in three domains: \textit{Card Flip}, \textit{Bookshelf}, and \textit{Kitchen} (Figure~\ref{fig:CPNP_tasks}). Each domain is equipped with a skill library $\mathcal{K}$. In the Card Flip domain, the skill library is $ \mathcal{K}=\{K_{\text{slide}}, K_{\text{prehensile}}\}$, where $K_{\text{slide}}$ slides the card on the table. In the Bookshelf domain, $\mathcal{K} = \{K_{\text{topple}}, K_{\text{push}}, K_{\text{prehensile}}\}$, where $K_{\text{topple}}$ topples books on the upper shelf to expose graspable poses, $K_{\text{push}}$ slides books on the lower shelf. In the Kitchen domain, $\mathcal{K}_{\text{kitchen}} = \{K_{\text{sink}}, K_{\text{cupboard}}, K_{\text{prehensile}}\}$, where $K_{\text{sink}}$ and $K_{\text{cupboard}}$ are non-prehensile skills that manipulates objects to the target pose in the sink and the cupboard respectively. In all domains, $K_{\text{prehensile}}$ is a pick-and-place skill that moves an object from its current pose to the target pose. In all domains, initial and goal object poses are sampled from separate regions where no single skill suffices, requiring composition of multiple skills to reach the goal. See Appendix~\ref{Appendix:region} for details of our problem distribution.

We compare our method with the following baselines:
\begin{itemize}[leftmargin=10pt, itemsep=0.5pt]
    \item PPO~\cite{schulman2017proximal}: An RL method that directly outputs joint torque commands along with joint gain and damping values without utilizing a pre-trained skills $\mathcal{K}$. Trained with a reward function based on the distance between the current and goal object poses.
    \item \texttt{MAPLE}~\cite{nasiriany2022augmenting}: A state-of-the-art PAMDP RL method trained with a reward function that rewards the robot when the high-level policy selects a feasible skill, successfully completes the task, or reduces the distance between the current and goal object poses. Uses same set of pre-trained skills as our method.
    \item \texttt{HLPS}~\cite{wang2024probabilistic}: A state-of-the-art hierarchical RL method that, instead of using pre-trained skills, simultaneously learns low-level and high-level policies to achieve the goal. The high-level policy outputs a subgoal for a low-level policy, and is trained with the reward function based on the distance between the current and goal object pose. The low-level policy is trained with the reward function based on the distance to the subgoal provided by the high-level policy.
    \item \texttt{Skill-RRT}: Our planner without policy distillation.
    \item SPIN: Our method with the replay success threshold of $m=0.9$
    %\item Ours-w/o-\texttt{filtering}: Imitation learning using demonstrations from \texttt{Skill-RRT} without filtering, used to train each model for each domain.
\end{itemize}
The summary of these baselines is presented in the first two columns of Table~\ref{table:main_exp}. The details for how we train these baselines and their MDP definitions are included in Appendix Appendix~\ref{Appendix:baseline_PPO}, ~\ref{Appendix:baseline_MAPLE}, and ~\ref{Appendix:baseline_HLPS}. For each baseline, we report the number of state-action pairs used for training across the three domains in Table~\ref{table:data_summary}. 

\input{tables/main_exp}

Table~\ref{table:main_exp} shows the results of these methods across the three domains. PPO, which does not use temporally-abstracted actions, failed to solve the problems for all domains, because the tasks were too long-horizon (up to 564 number of low-level actions) for the agent to achieve task success and falls into a local optima. \texttt{HLPS}, which simultaneously learns to do the task and discover low-level policies, also achieves zero task success in all domains because of the fundamental problem with hierarchical RL: the high-level policy must adapt to the evolving low-level policy. \texttt{MAPLE}, on the other hand, leverages the pre-trained skills $\mathcal{K}$, and achieves 78\% in the bookshelf domain. However, in two other domains that narrow passages, where there is a much narrower set of intermediate object poses that the robot must go through to achieve the goal, such as the edge of the table for the Card Flip domain, it achieves zero success rates (see Appendix Figure~\ref{fig:card_y_position_histograms} for a visual illustration).  


It struggles in these domains due to the narrow passage problem~\cite{hsu1998finding}. For instance, in the Card Flip domain, the card can only be flipped near the edges of the table, which constitute a very small region in $\Qobj$. Moreover, even at the edge, to prevent the card from dropping during the transition from sliding to the prehensile skill, the card must be positioned precisely: it must be graspable while remaining sufficiently close to the table surface to avoid falling during the transition 


Similarly, in the Kitchen domain, the robot must position the cup such that the prehensile skill can be applied following the non-prehensile skill in the sink. The set of cup poses suitable for applying the prehensile skill is very narrow: the pose must be collision-free, and a valid inverse kinematics solution must exist. As a result, most attempts at exploring object subgoal poses lead to failure for \texttt{MAPLE}, which ends up learning only locally optimal behaviors, such as bringing the card to the edge of the table but avoiding the prehensile action to prevent the card from falling. In the Bookshelf domain, where the robot simply needs to topple the book to enable grasping, \texttt{MAPLE} achieves an 83\% success rate.

In contrast, \texttt{Skill-RRT} avoids these limitations through two key advantages. First, unlike RL methods such as \texttt{MAPLE}, which often converge to locally optimal behaviors to avoid failure (e.g., leaving the card safely on the table without attempting the flip), \texttt{Skill-RRT} persistently explores skill sequences and subgoal object poses via RRT-based search. This prevents it from getting trapped in local minima: even when sampled plans fail, the planner continues exploring until a successful sequence is found. Second, \texttt{Skill-RRT} can discover feasible subgoal regions that are extremely narrow and difficult to find through random exploration. For example, in the kitchen domain, graspable and collision-free cup poses are rare and require precise non-prehensile manipulation beforehand. While \texttt{MAPLE} struggles to reach such subgoals due to the limitations of reward-driven exploration, \texttt{Skill-RRT}'s RRT-based exhaustive search strategy enables it to identify and reach these critical subgoal configurations, resulting in successful task completions across challenging domains. While \texttt{Skill-RRT} successfully finds solutions in all domains, achieving 39\% success in Card Flip, 66\% in Bookshelf, and 64\% in Kitchen, it still faces limitations for real-world deployment. They remain insufficient for practical use without further refinement. In addition, planning can take up to 120 seconds, making the approach less suitable for time-sensitive applications.

To overcome the limitations of \texttt{Skill-RRT}, we distill a policy from successful trajectories generated by \texttt{Skill-RRT}, and refer to this baseline as \texttt{Ours-w/o-filtering}. \texttt{Skill-RRT} executes a single skill plan, which makes it vulnerable to deviations from the expected state during execution. In contrast, the distilled policy is trained on a diverse set of successful demonstrations from multiple skill plans generated by \texttt{Skill-RRT}. As a result, it can generalize to similar but not identical states and recover from small deviations, leading to higher robustness and improved overall success rates compared to directly replaying a single skill plan. Empirically, \texttt{Ours-w/o-filtering} achieves 82\% success in Card Flip, 83\% in Bookshelf, and 87\% in Kitchen, while reducing the computation time to within 3 seconds, making real-world deployment feasible. However, there is still room for improvement, as the success rates remain below perfect reliability.

To further improve the robustness of the distilled policy, we introduce a skill plan filtering method that removes risky demonstrations before imitation learning. Specifically, we eliminate skill plans that succeed once but are highly sensitive to small deviations, such as placing the card near the edge of the table in the Card Flip domain. Although such demonstrations can succeed under ideal conditions, slight errors during execution often lead to failure, such as the card falling off the table. By filtering out these unstable intermediate skill goals, the policy is distilled from robust and reproducible skill sequences, resulting in improved generalization and execution stability. As a result, our final policy (\texttt{Skill-RRT}+\texttt{filtering}+IL) achieves over 90\% success rates across all domains in simulation, while maintaining a computation time of less than 3 seconds, making it feasible for real-world deployment. Additional details of the filtering method are provided in Appendix~\ref{Appendix:data_qual}.

\subsection{Real World Experiments}
We evaluate our distilled policy in the real world by zero-shot transferring the policy trained in simulation. For each experiment, we use a set of 20 test problems consisting of different initial object poses, initial robot configurations, and goal object poses. The shapes of the real environments and objects are identical to those in simulation. Our policy achieves 85\% (17/20), 90\% (18/20) and 80\% (16/20) in the card flip, bookshelf, and kitchen domains respectively.

There are nine failures in total across the three domains, and they can be categorized into three cases. The first case involves unexpected contacts between the robot and the object during NP manipulations, which drive the object into out‑of‑distribution states (55.6\%). In the kitchen domain, for example, an unintended collision between the cup and the robot causes the cup to become trapped against the sink wall, preventing the robot from reaching the desired grasp position. The second case results from hardware torque limit violations, caused by excessive impacts during NP manipulations, such as a strong collision with the table in the card domain (22.2\%). The third case arises from in‑hand object disturbance during placement, due to collisions between the object and the environment (22.2\%). For instance, while placing a book into a narrow space of the lower shelf, the book collide with the box.


%Our policy achieves a success rate of over 80\% across all domains within a reasonable amount of execution time: Card Flip, Bookshelf, Kitchen domains take 40.2, 56.3, and 72.5 seconds on average, respectively, as shown in Table~\ref{table:real_world_result}.

\iffalse
\begin{wraptable}{r}{0.6\textwidth}
% \vspace{-1em}
\centering
\setlength\tabcolsep{10pt}
\renewcommand{\arraystretch}{1.2}
\begin{adjustbox}{width=0.5\textwidth}
\begin{tabular}{cccc}
\toprule
& \textbf{Card Flip} & \textbf{Bookshelf} & \textbf{Kitchen} \\
\midrule
\makecell{Success rate (\%) \\ (Success/Trials)}  &  85 (17/20)   & 90 (18/20)   &  80 (16/20) \\
% \midrule
% Solving Time (s)  &  40.2   & 56.3   &  72.5 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Real-world experimental results on three domains.}
\label{table:real_world_result}
\vspace{-1em}
\end{wraptable}
\fi


We conduct additional ablation studies to validate the design choices of our framework. Specifically, we investigate three aspects: (1) the necessity of learning the \textit{connector}; (2) the importance of the \textit{data filtering} method during IL with qualitative analysis; and (3) the impact of different \textit{model architectures} on IL performance. Due to space limitations, detailed results and analyses are provided in Appendix~\ref{Appendix:Ablation}.


% \input{tables/real_world_result}

\iffalse
\subsection{Ablation Studies}
\fi

==> sections/05_ablation.tex <==
\subsection{Motivation of connectors}
We use reinforcement learning (RL) policies, called connectors, to generate smooth transitions between the end of one skill and the start of the next. This is necessary because our skills are trained independently and often leave gaps in object or robot state. While a standard motion planner such as Bi-RRT from OMPL~\cite{sucan2012the-open-motion-planning-library} could also be used to fill these gaps, we find that RL-based connectors are more effective for two reasons. First, they achieve higher success rates in transitions that involve contact changes between the robot and object. Second, they offer much faster inference than sampling-based planners, which helps accelerate our overall skill composition method, \texttt{Skill-RRT}. The robustness of our connectors, as compared to the motion planner, and supporting evidence for the claims above are provided in Appendix~\ref{Appendix:Connector_vs_MP}.

\subsection{Ablation on Imitation Learning Architectures}
We adopt a diffusion policy to handle the multi-modality of imitation learning data. To validate this design choice, we compare it with four alternative architectures commonly used in imitation learning: ResNet~\cite{he2016deep}, LSTM+GMM~\cite{robomimic2021}, conditional VAE (cVAE)\cite{kingma2013auto}, and Transformer\cite{vaswani2017attention}. All models are trained on the same dataset with approximately 70M parameters and identical training settings.

As shown in Table~\ref{table:IL_arch_ablation}, the diffusion policy achieves the highest success rate in the card flip domain, where the diversity of intermediate object poses is high. In the bookshelf and kitchen domains, where such diversity is lower, other architectures perform comparably well. cVAE consistently underperforms, suggesting that the smoothing effect of VAE harms task-specific precision. These results indicate that diffusion policy is particularly beneficial in tasks requiring accurate modeling of diverse multimodal behaviors. Details on training setups are provided in Appendix~\ref{Appendix:IL_arch_ablation}.

==> tables/experiment/exp_setup.tex <==
\begin{table*}[ht]
\vspace{-5mm}
\centering
\renewcommand{\arraystretch}{1.5} % Adjust row spacing
\begin{adjustbox}{width=1.7\columnwidth}
% \setlength\tabcolsep{20 pt}
\begin{tabular}{|c|c|c|c|}
\hline
  & \textbf{Card Flip} & \textbf{Bookshelf} & \textbf{Kitchen} \\
\hline
object pose space $\Qobj$ & $R^\text{up} \cup R^\text{down}$ & $R^\text{uppershelf} \cup R^\text{lowershelf}$ &  $ R^\text{sink} \cup R^\text{leftshelf} \cup R^\text{rightshelf}$ \\
\hline
set of skills $\mathcal{K}$ & $\{K_\text{P}, K_{\text{NP}_{\text{up}}}, K_{\text{NP}_{\text{down}}}\}$ & $\{K_\text{P}, K_{\text{NP}_{\text{topple}}}, K_{\text{NP}_{\text{push}}}\}$ & $\{K_\text{P}, K_{\text{NP}_\text{sink}}, K_{\text{NP}_\text{leftshelf}},  K_{\text{NP}_\text{rightshelf}}\}$ \\
\hline
\end{tabular}
\end{adjustbox}
\begin{flushleft}
\footnotesize
\caption{Experimental setup of object pose space $\Qobj$, and a set of skills $\mathcal{K}$ for each domain.}\label{table:exp_setup}
\end{flushleft}
\vspace{-6mm}
\end{table*}


==> tables/notations/IL.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=\columnwidth} % Automatically fit within column width
\begin{tabular}{|c|p{0.75\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline

$\theta$ & Replay success rate threshold \\ \hline
$\pi_{\text{IL}}$ & Imitation learned policy \\ \hline
$\mathcal{D}_{\text{imitate}}$ & Dataset consisting of state-action pairs from the replay of skill plans $\tau_{\text{skill}}$ \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Notation table for imitation learning}
\label{tab:IL_notation}
\end{table}

==> tables/notations/connector.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=\columnwidth} % Automatically fit within column width
\begin{tabular}{|c|p{0.75\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline

$c_\alpha$ & connector skill for skill $o_\alpha$ \\ \hline
$C$ & connector library contatining all connectors $C = \{c_{\text{NP}_1}, c_{\text{NP}_2}, \dots, c_{\text{Place}}\}$ \\ \hline
$\tau_{\text{skill}}^\text{abstract}$ & An abstract skill plan that consists solely of a sequence of skills and their associated subgoals, excluding any connector information. \\ \hline
$r^{\text{ee}}$ & End-effector distance reward: encourages the end-effector to move closer to its target position \\ \hline
$r^{\text{tip}}$ & Gripper tip position reward: aligns the gripper tips with their target positions \\ \hline
$r^{\text{success}}$ & Success reward: awarded when both the end-effector pose and gripper tip reach their target positions successfully \\ \hline
$r^{\text{object\_vel}}$ & Object velocity penalty: penalizes unnecessary object movement to maintain the validity of subsequent skill preconditions \\ \hline
$\epsilon^{\text{ee}}_0, \epsilon^{\text{ee}}_1$ & Parameters for the end-effector distance reward \\ \hline
$\epsilon^{\text{tip}}_0, \epsilon^{\text{tip}}_1$ & Parameters for the gripper tip position reward \\ \hline
$w^{\text{vel}}$ & Weight parameter for the object velocity penalty \\ \hline
$x_t^{\text{ee}}$ & End-effector keypoints at timestep $t$ \\ \hline
$\mathbf{x}_g^{\text{ee}}$ & Subgoal end-effector keypoints \\ \hline
$\mathbf{x}_t^{\text{tip}}$ & Gripper tip position at timestep $t$ \\ \hline
$\mathbf{x}_g^{\text{tip}}$ & Subgoal gripper tip position \\ \hline
$\mathbf{x}_t^{\text{obj}}$ & Object keypoints at timestep $t$ \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Notation table for connector}
\label{tab:connector_notation}
\end{table}


==> tables/notations/skill-rrt.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=\columnwidth} % Automatically fit within column width
\begin{tabular}{|c|p{0.75\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline

$d$ & Metric function which calculates the distance between two object poses $q^{\text{obj}}$ and $q^{\text{obj}}_{\text{sg}}$ \\ \hline
$p_g$ & Goal object pose sampling probability during skill-RRT \\ \hline
$N_{max}$ & Maximum number of extend nodes to the tree during skill-RRT \\ \hline
$T$ & Tree in skill-RRT \\ \hline
$v$ & Node in the tree \\ \hline
$e$ & Edge in the tree \\ \hline
$T.V$ & Set of nodes in the tree $T$ \\ \hline
$v_0$ & Initial node \\ \hline
$v_{\text{near}}$ & Nearest node to the new node \\ \hline
$v_{\text{new}}$ & Newly added node \\ \hline
$v_{\text{goal}}$ & Node where the goal object pose serves as its subgoal object pose \\ \hline
$e_{\text{new}}$ & Newly added edge \\ \hline
$v.q^{\text{obj}}$ & Object pose at the node \\ \hline
$v.q^{\text{robot}}$ & Robot configuration at the node \\ \hline
$v.q^{\text{obj}}_{\text{sg}}$ & Subgoal object pose at the node \\ \hline
$\texttt{simulate}$ & Simulation function (IsaacGym) \\ \hline
$\tau_{\text{skill}}$ & Skill plan, consisting of a sequence of skills, connectors and their subgoals \\ \hline
$o_k$ & $k$-th skill in the skill plan $\tau_{\text{skill}}$ \\ \hline
$v_k$ & $k$-th node in the sequence of nodes from $v_0$ to $v_\text{goal}$ \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Notation table for SKILL-RRT}
\label{tab:skillrrt_notation}
\end{table}

==> tables/notations/skill.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=\columnwidth} % Automatically fit within column width
\begin{tabular}{|c|p{0.75\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline

$\mathcal{O}$ & Skill library containing all skills: $\mathcal{K} = \{o_{\text{NP}_1}, \dots, o_{\text{NP}_n}, o_{\text{Place}}\}$ \\ \hline
$i \in \{1, 2, \dots, n\}$ & Index for Non-Prehensile skills \\ \hline
$\alpha \in \{\text{NP}_1, \text{NP}_2, \dots, \text{NP}_n, \text{Place}\}$ & Index for skills in the skill library \\ \hline
$o_{\text{NP}_i}$ & $i$-th Non-Prehensile skill for manipulating objects in region $\mu_i$ \\ \hline
$o_{\text{Place}}$ & Skill for placing the object between different regions \\ \hline
% $\mu^i \subset SE(2)$ & Set of object poses manipulated by the $i$-th Non-Prehensile skill $o_{\text{NP}_i}$ \\ \hline
$\mu^i_\mathcal{I} \subset SE(2)$ & Set of initial object poses manipulated by the $i$-th Non-Prehensile skill $o_{\text{NP}_i}$ \\ \hline
$\mu^i_\beta \subset SE(2)$ & Set of subgoal object poses manipulated by the $i$-th Non-Prehensile skill $o_{\text{NP}_i}$ \\ \hline
$\mathcal{M}$ & Set of regions: $\mathcal{M} = \{(\mu^1_{\mathcal{I}}, \mu^1_\beta), (\mu^2_{\mathcal{I}}, \mu^2_\beta), \dots, (\mu^n_{\mathcal{I}}, \mu^n_\beta) \}$ \\ \hline
$\pi_\alpha(a \mid s, q^{\text{obj}}_\text{sg})$ & Policy function for generating actions based on the current and subgoal states of skill $o_\alpha$\\ \hline
$f_\alpha^{\text{pre}}(q^{\text{obj}}, q^{\text{obj}}_\text{sg})$ & Pre-contact Robot Configuration Sampler of skill $o_\alpha$ \\ \hline
$q^{\text{robot}}_{\text{pre}}$ & Pre-contact robot configuration \\ \hline
$\mathrm{pre}^{\text{level}}_\alpha(q^{\text{obj}}, q^{\text{robot}}, q^{\text{obj}}_{\text{sg}})$ & Precondition function for the skill $o_\alpha$ that takes $q^{\text{obj}}$, $q^{\text{robot}}$, and $q^{\text{obj}}_{\text{sg}}$ with abstract level \\ \hline
$c_\alpha$ & Connector for skill $o_\alpha$ \\ \hline
$\pi^c_\alpha(a \mid s, q^{\text{robot}}_{\text{sg}})$ & Policy function that generates actions for the connector $c_\alpha$, given $s$, and $q^{\text{robot}}_\text{sg}$ \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Notation table for skill}
\label{tab:skill_notation}
\end{table}


==> tables/notations/skill_train.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=0.5\textwidth} % Adjusts the table width to half the page

\begin{tabular}{|c|p{0.5\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline

$r^{\text{object}}$ & Object keypoint distance reward: encourages moving the object closer to its target subgoal object pose \\ \hline
$r^{\text{tip-object}}$ & Tip contact reward: maintain contact between the gripper tips and the object \\ \hline
$r^{\text{rotation}}$ & Object rotation reward: encourages moving the object's quaternion to its target subgoal object quaternion \\ \hline
$r^{\text{grasp}}$ & Relative grasp reward: Ensure the gripper tips
maintain a grasp on the object \\ \hline
$r^{\text{success}}$ & Success reward: awarded when both the end-effector pose and gripper tip reach their target positions successfully \\ \hline
$\epsilon^{\text{object}}_0, \epsilon^{\text{object}}_1$ & Parameters for the object keypoint distance reward \\ \hline
$\epsilon^{\text{tip-object}}_0, \epsilon^{\text{tip-object}}_1$ & Parameters for the tip contact reward \\ \hline
$w^{\text{grasp}}$ & Weight parameter for the relative grasp reward \\ \hline
$x_t^{\text{ee}}$ & End-effector keypoints at timestep $t$ \\ \hline
$x_g^{\text{ee}}$ & Subgoal end-effector keypoints \\ \hline
$x_t^{\text{tip}}$ & Gripper tip position at timestep $t$ \\ \hline
$x_t^{\text{object}}$ & Object keypoints at timestep $t$ \\ \hline
$x_g^{\text{object}}$ & Goal Object keypoints (object keypoints of subgoal object pose) \\ \hline
$h_t^{\text{object}}$ & Object quaternion at timestep $t$ \\ \hline
$h_g^{\text{object}}$ & Goal object quaternion \\ \hline

$q_t^{O}$ & Object Pose at timestep $t$ \\ \hline
$\mathtt{rel}(a, b)$ & Function to calculate the relative position of $a$ with respect to pose $b$ \\ \hline

\end{tabular}
\end{adjustbox}
\caption{Notation table for skill training}
\label{tab:connector_notation}
\end{table}


==> tables/notations/state.tex <==
\begin{table}[h!]
\large
\centering
\begin{adjustbox}{width=\columnwidth} % Automatically fit within column width
\begin{tabular}{|c|p{0.75\columnwidth}|} % Adjust the second column width proportionally
\hline
\textbf{Symbol} & \textbf{Explanation} \\ \hline
$q^{\text{obj}} \in SE(2)$ & Object pose \\ \hline
$q^{\text{robot}} \in \mathbb{R}^9$ & Robot configuration (9 DoF robot joint position) \\ \hline
$q^{\text{obj}}_\text{sg} \in SE(2)$ & Subgoal object pose \\ \hline
$q^{\text{robot}}_\text{sg} \in SE(3) \times \mathbb{R}^3$ & Subgoal robot configuration (End-effector pose in $SE(3)$ and gripper tip positions in 3D space) \\ \hline
$q^{\text{obj}}_{\text{init}} \in SE(2)$ & Initial object pose of the task \\ \hline
$q^{\text{robot}}_{\text{init}} \in \mathbb{R}^9$ & Initial robot configuration of the task (9 DoF robot joint position) \\ \hline
$q^{\text{obj}}_{\text{goal}} \in SE(2)$ & Goal object pose of the task \\ \hline
$s$ & State \\ \hline
% $sg$ & Subgoal information (e.g., subgoal object pose, robot configuration) \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Notation table for task parameters}
\label{tab:state_notation}
\end{table}


==> tables/object_figure.tex <==
% \begin{table}[ht]
% \centering
% \caption{Objects Images in Simulation and Real World}
% \begin{adjustbox}{max width=\textwidth}
% \begin{tabular}{|>{\centering\arraybackslash}m{0.1\textwidth}|>{\centering\arraybackslash}m{0.3\textwidth}|>{\centering\arraybackslash}m{0.3\textwidth}|}
% \hline
% \textbf{Object} & \textbf{Simulation} & \textbf{Real World} \\
% \hline
% \textbf{Card} & \includegraphics[width=0.25\textwidth]{figures/object/sim_card.png} & \includegraphics[width=0.25\textwidth]{figures/object/real_card.jpg} \\
% \hline
% \textbf{Book} & \includegraphics[width=0.25\textwidth]{figures/object/sim_book.png} & \includegraphics[width=0.25\textwidth]{figures/object/real_book.jpg} \\
% \hline
% \textbf{Cup} & \includegraphics[width=0.25\textwidth]{figures/object/sim_cup.png} & \includegraphics[width=0.25\textwidth]{figures/object/real_cup.jpg} \\
% \hline
% \end{tabular}
% \end{adjustbox}
% \label{tab:objects_sim_real}
% \end{table}

\begin{table}[ht]
\centering
\small
\caption{Objects Images in Simulation and Real World}
\begin{adjustbox}{max width=0.9\textwidth}
\begin{tabular}{|>{\centering\arraybackslash}m{0.1\textwidth}|>{\centering\arraybackslash}m{0.3\textwidth}|>{\centering\arraybackslash}m{0.3\textwidth}|>{\centering\arraybackslash}m{0.3\textwidth}|}
\hline
\textbf{Object} & \textbf{Card} & \textbf{Book} & \textbf{Cup} \\
\hline
\textbf{Simulation} & \includegraphics[width=0.25\textwidth]{figures/object/sim_card_white_background.png} & \includegraphics[width=0.25\textwidth]{figures/object/sim_book.png} & \includegraphics[width=0.25\textwidth]{figures/object/sim_cup.png} \\
\hline
\textbf{Real} & \includegraphics[width=0.25\textwidth]{figures/object/real_card_white_background.png} & \includegraphics[width=0.25\textwidth]{figures/object/real_book_white_background.png} & \includegraphics[width=0.25\textwidth]{figures/object/real_cup_white_backgound.png} \\
\hline
\end{tabular}
\end{adjustbox}
\label{tab:objects_sim_real}
\end{table}

==> tables/real_world_result.tex <==
\begin{table}[ht]
\centering
\setlength\tabcolsep{10 pt}
% \begin{adjustbox}{max width=\columnwidth}
\begin{tabular}{cccc}
\toprule
           & \textbf{Card Flip} & \textbf{Bookshelf} & \textbf{Kitchen} \\
\midrule
\makecell{Success rate (\%) \\ (Success/Trials)}  &  85 (17/20)   & 90 (18/20)   &  80 (16/20) \\
\midrule
Solving Time (s)  &  \textcolor{red}{10}   & \textcolor{red}{10}   &  \textcolor{red}{10} \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\caption{Real-world experimental results on three domains.}
\label{table:real_world_result}
\end{table}
